Wavenumber-explicit stability and convergence analysis of hp finite element discretizations of Helmholtz problems in piecewise smooth media

We present a wavenumber-explicit convergence analysis of the hp finite element method applied to a class of heterogeneous Helmholtz problems with piecewise analytic coefficients at large wavenumber $k$. Our analysis covers the heterogeneous Helmholtz equation with Robin, exact Dirichlet-to-Neumann, and second order absorbing boundary conditions, as well as perfectly matched layers.

==> 00_notes.tex <==
% !TEX root = main.tex
\section{Notes}\label{section:notes}

We consider the following Helmholtz problem:
\begin{equation}\label{eq:heterogeneous_helmholtz_boundary_value_problem}
	\begin{alignedat}{2}
		- \Delta u - k^2 n^2(x) u &= f \quad   &&\text{in } \Omega,\\
		\partial_n u - i k u      &= 0         &&\text{on } \partial \Omega.
	\end{alignedat}
\end{equation}
Throughout this paper, if not otherwise stated, we assume the following:
\begin{assumption}\label{assumption:general_assumptions}
	In spatial dimension $d = 2,3$ the bounded Lipschitz domain $\Omega \subset \mathbb{R}^d$ has an analytic boundary $\partial \Omega$.
  The wavenumber $k$ satisfies $ k \geq k_0 > 0 $.
  Furthermore, the spatial dependent heterogeneity $n$ is analytic on $\overline{\Omega}$ or piecewise analytic with an analytic interface $\Gamma_i$.
	In the case of piecewise analyticity we assume the interface and the boundary of $\Omega$ to be separated, i.e., $\mathrm{dist}(\Gamma_i, \partial \Omega) > 0$.
	Furthermore, $n$ is uniformly bounded, i.e.
  \begin{equation*}
    0 < c_{\min} \leq n(x) \leq c_{\max}, \qquad \forall x \in \Omega.
  \end{equation*}
	and satisfies the analyticity estimate
	\begin{equation*}
    \lVert \nabla^p ( n^2 ) \rVert_{L^\infty(\omega)} \leq C_n \gamma_n^p p!, \qquad \forall p \in \mathbb{N}_0,
  \end{equation*}
	for some constants $C_n \geq 0$ and $\gamma_n \geq 0$, where $\omega$ is either $\Omega$ or  $\Omega \setminus \Gamma_i$.
  The data $f$ satisfies $f \in L^2(\Omega)$.
	Regarding unique solvability, we assume problem \eqref{eq:heterogeneous_helmholtz_boundary_value_problem} to be well posed, i.e., it admits a unique weak solution $u \in H^1(\Omega)$ and the \textit{a priori} energy bound
	\begin{equation}\label{eq:stability_estimate}
		\lVert \nabla u \rVert_{L^2(\Omega)} + k \lVert u \rVert_{L^2(\Omega)} \leq \StabilityConstant \lVert f \rVert_{L^2(\Omega)},
	\end{equation}
	holds with a constant $\StabilityConstant$.
\end{assumption}
Regarding the stability constant $\StabilityConstant$ see also \cite{barucq-chaumont-frelet-gout17, graham-sauter20} for further discussion.
\TCF{Can you point towards any other important references regarding stability estimates?}
If not otherwise stated we furthermore assume polynomial well-posedness of the problem:
\begin{assumption}[Polynomial well-posedness]
	The solution operator $f \mapsto u$ grows only polynomially in the wavenumber $k$, i.e.,
	\begin{equation*}
		\StabilityConstant \lesssim k^\alpha
	\end{equation*}
	for some $\alpha \geq 0$.
\end{assumption}
Assumption \ref{assumption:general_assumptions} allows to consider, without loss of generality, the problem
\begin{equation}\label{eq:heterogeneous_helmholtz_boundary_value_problem_new}
	\begin{alignedat}{2}
		- \Delta u - k^2 n^2 u &= n^2 f \quad   &&\text{in } \Omega,\\
		\partial_n u - i k u   &= 0         &&\text{on } \partial \Omega.
	\end{alignedat}
\end{equation}
Since the $\lVert f \rVert_{L^2(\Omega)} \simeq \lVert n f \rVert_{L^2(\Omega)}$.
In the following we develop analogous high and low pass filters introduced in \cite{melenk-sauter10, melenk-sauter11} appropriate for the heterogeneous Helmholtz equation.
For the homogeneous Helmholtz equation the main tool is the Fourier transform.
For the heterogeneous version we are going to expand a given function in $L^2(\Omega)$ into a problem adapted Fourier series.
The low and high pass filters will then be given as the low and high frequency part of the Fourier expansion respectively.
To that end consider the following eigenvalue problem for the eigenpairs $(\varphi_i, \lambda_i^2)_{i \in \mathbb{N}}$
\begin{equation}\label{eq:heterogeneuos_eigenvalue_problem}
	\begin{alignedat}{2}
		  - \Delta \varphi_i  &= \lambda_i^2 n^2 \varphi_i \quad   &&\text{in } \Omega,\\
	   \partial_n \varphi_i &= 0                                 &&\text{on } \partial \Omega.
	\end{alignedat}
\end{equation}
We introduce the space $L^2(\Omega, n)$ as the space of square integrable functions with the weighted $L^2$-inner product and norm given by
\begin{equation*}
  (u, v)_{L^2(\Omega, n)} \coloneqq \int_\Omega u(x) \overline{v}(x) n^2(x) dx, \quad \lVert u \rVert_{L^2(\Omega, n)} \coloneqq (u, u)_{L^2(\Omega, n)}^{1/2}.
\end{equation*}
Note that due to Assumption \ref{assumption:general_assumptions} we have
\begin{equation*}
  c_{\min} \lVert u \lVert_{L^2(\Omega)} \leq \lVert u \lVert_{L^2(\Omega, n)} \leq c_{\max} \lVert u \lVert_{L^2(\Omega)},
\end{equation*}
i.e. the spaces $L^2(\Omega, n)$ and $L^2(\Omega)$ are the same up to equivalent norms.
Furthermore, let $L_0^2(\Omega, n)$ denote the space of all $f \in L^2(\Omega, n)$, such that $\int_\Omega f n^2 dx = 0$.
We solve the eigenvalue problem \eqref{eq:heterogeneuos_eigenvalue_problem} on the space $H^1(\Omega) \cap L^2_0(\Omega, n)$.
Let $S: L_0^2(\Omega, n) \rightarrow L_0^2(\Omega, n)$ be the solution operator of the problem
\begin{equation*}
	\begin{alignedat}{2}
		  - \Delta u &= n^2 f \quad   &&\text{in } \Omega,\\
			\partial_n u &= 0           &&\text{on } \partial \Omega,
	\end{alignedat}
\end{equation*}
mapping $f \in L_0^2(\Omega, n)$ to the corresponding weak solution $u = Sf$, i.e., $u \in H^1(\Omega) \cap L^2_0(\Omega, n)$ satisfies
\begin{equation*}
	(\nabla u, \nabla v) = (f, v)_{L^2(\Omega, n)}, \quad \forall v \in H^1(\Omega) \cap L^2_0(\Omega, n).
\end{equation*}
Regarding unique solvability, note that the space $H^1(\Omega) \cap L^2_0(\Omega, n)$ is a Hilbert space since it is the kernel of the continuous linear functional $H^1(\Omega) \ni f \mapsto \int_\Omega f n^2 dx \in \mathbb{R}$.
Furthermore, $\norm{\nabla u}_{L^2(\Omega)}$ is an equivalent norm on $H^1(\Omega) \cap L^2_0(\Omega, n)$.
Therefore, unique solvability of the weak formulation as well as continuity of the solution operator $S$ follows by Lax-Milgram.
Due to compact embedding of $H^1(\Omega) \cap L^2_0(\Omega, n)$ into $L^2_0(\Omega, n)$ the operator $S$ is in fact compact.
Furthermore, it is easily checked that $S$ is symmetric and positive.
Therefore, standard spectral theory gives the existence of eigenpairs $(\varphi_i, \lambda_i^2)_{i \in \mathbb{N}}$.
Finally, since the eigenpairs satisfy
\begin{equation*}\label{eq:weak_formulation_heterogeneous_eigenvalue_problem}
	(\nabla \varphi_i, \nabla v) = \lambda_i^2 (\varphi_i, v)_{L^2(\Omega, n)}, \quad \forall v \in H^1(\Omega) \cap L^2_0(\Omega, n)
\end{equation*}
choosing $v = \varphi_j$ gives
\begin{equation*}
	(\nabla \varphi_i, \nabla \varphi_j) = \lambda_i^2 (\varphi_i, \varphi_j)_{L^2(\Omega, n)} = \lambda_i^2 \delta_{ij}.
\end{equation*}
Therefore, the orthonormal basis $(\varphi_i)_{i \in \mathbb{N}}$ is also orthogonal with respect to the inner product $(\nabla u , \nabla v)$ and we have $\norm{\nabla \varphi_i}_{L^2(\Omega)} = \lambda_i$.
Note that the weak formulation \eqref{eq:weak_formulation_heterogeneous_eigenvalue_problem} is actually satisfied for all $v \in H^1(\Omega)$.
Writing $v = v_\Omega + \tilde{v}$ with $v_\Omega$ being the weighted integral mean and $\tilde{v} \in H^1(\Omega) \cap L^2_0(\Omega, n)$ we find
\begin{equation*}
	(\nabla \varphi_i, \nabla v)
	= (\nabla \varphi_i, \nabla \tilde{v})
	= \lambda_i^2 (\varphi_i, \tilde{v})_{L^2(\Omega, n)}
	= \lambda_i^2 (\varphi_i, \tilde{v})_{L^2(\Omega, n)} + \lambda_i^2 \underbrace{(\varphi_i, v_\Omega)_{L^2(\Omega, n)}}_{=0}
	= \lambda_i^2 (\varphi_i, v)_{L^2(\Omega, n)}.
\end{equation*}
We add the constant function, corresponding to the zero eigenvalue, to the orthonormal basis $(\varphi_i)_{i \in \mathbb{N}}$ again denoting it by $(\varphi_i)_{i \in \mathbb{N}}$.
The new system $(\varphi_i)_{i \in \mathbb{N}}$ is an orthonormal basis of $L^2(\Omega, n)$ and is still orthogonal with respect to the inner product $(\nabla u , \nabla v)$.
We have therefore proven the following
\begin{theorem}[Properties of eigenpairs of problem \eqref{eq:heterogeneuos_eigenvalue_problem}]\label{theorem:results_on_eigenfunctions}
	Let $\Omega$ be a bounded Lipschitz domain and $n$ uniformly bounded on $\overline{\Omega}$.
	Then there exists an $L^2(\Omega, n)$ orthonormal basis $(\varphi_i)_{i \in \mathbb{N}}$ consisting of the eigenpairs $(\varphi_i, \lambda_i^2)_{i \in \mathbb{N}}$ corresponding to problem \eqref{eq:heterogeneuos_eigenvalue_problem}.
	The eigenfunctions are also orthogonal with respect to the inner product $(\nabla \cdot, \nabla \cdot)$ and satisfy $\norm{\nabla \varphi_i}_{L^2(\Omega)} = \lambda_i$.
	Finally, any $f \in L^2(\Omega,n)$ can be expanded into a Fourier series and the Parseval identity holds, i.e.,
	\begin{equation*}
		f = \sum_{i \in \mathbb{N}} f_i \varphi_i, \qquad f_i = (f, \varphi_i)_{L^2(\Omega, n)} , \qquad 	\lVert f \rVert_{L^2(\Omega, n)}^2 = \sum_{i \in \mathbb{N}} |f_i|^2,
	\end{equation*}
	where the series converges in $L^2(\Omega, n)$.
\end{theorem}
We relate summability of the Fourier coefficients to Sobolov regularity.
\begin{lemma}[Connection between summability of Fourier coefficients and regularity]\label{lemma:connection_summability_regularity}
	Let $\Omega$ be a bounded Lipschitz domain and $n$ uniformly bounded on $\overline{\Omega}$.
	For $f \in L^2(\Omega, n)$ there holds:
	\begin{enumerate}
		\item \label{item:summability_L2} $\lVert f \rVert_{L^2(\Omega)}^2 \simeq \lVert f \rVert_{L^2(\Omega, n)}^2 = \sum_{i \in \mathbb{N}} |f_i|^2$.
		\item \label{item:summability_H1} If $\sum_{i \in \mathbb{N}} |f_i|^2 \lambda_i^2 < \infty$ then $f \in H^1(\Omega)$. Furthermore,
		\begin{equation*}
			\nabla f =  \sum_{i \in \mathbb{N}} f_i \nabla \varphi_i,
			\qquad
			| f |_{H^1(\Omega)}^2 = \sum_{i \in \mathbb{N}} |f_i|^2 \lambda_i^2
			\qquad \text{and} \qquad
			\lVert f \rVert_{H^1(\Omega)}^2 \simeq \sum_{i \in \mathbb{N}} |f_i|^2 (1+\lambda_i^2).
		\end{equation*}
		Finally, for any $0 \leq s \leq 1$
		\begin{equation}\label{eq:interpolation_L2_H1}
			\lVert f \rVert_{H^s(\Omega)}^2 \simeq \sum_{i \in \mathbb{N}} |f_i|^2 (1 + \lambda_i^{2s}).
		\end{equation}
		If additionally $f \in L^2_0(\Omega, n)$ then
		\begin{equation*}
			\lVert f \rVert_{H^s(\Omega)}^2 \simeq \sum_{i \in \mathbb{N}} |f_i|^2 \lambda_i^{2s}.
		\end{equation*}
		\item \label{item:summability_H2} If $\partial \Omega$ is $C^2$ or $\Omega$ is a convex polygon, if $\sum_{i \in \mathbb{N}} |f_i|^2 \lambda_i^4 < \infty$ then $f \in H^2(\Omega)$ and $\partial_n f = 0$. Furthermore,
		\begin{equation*}
			\Delta f =  \sum_{i \in \mathbb{N}} f_i \Delta \varphi_i,
			\qquad
			| f |_{H^2(\Omega)}^2 \simeq \sum_{i \in \mathbb{N}} |f_i|^2 \lambda_i^4
			\qquad \text{and} \qquad
			\lVert f \rVert_{H^2(\Omega)}^2 \simeq \sum_{i \in \mathbb{N}} |f_i|^2 (1+\lambda_i^4).
		\end{equation*}
		Finally, for any $0 \leq s \leq 2$
		\begin{equation*}
			\lVert f \rVert_{H^s(\Omega)}^2 \simeq \sum_{i \in \mathbb{N}} |f_i|^2 (1 + \lambda_i^{2s}).
		\end{equation*}
		If additionally $f \in L^2_0(\Omega, n)$ then
		\begin{equation*}
			\lVert f \rVert_{H^s(\Omega)}^2 \simeq \sum_{i \in \mathbb{N}} |f_i|^2 \lambda_i^{2s}.
		\end{equation*}
	\end{enumerate}
\end{lemma}

\begin{proof}
	By norm equivalence and Parseval's identity assertion \ref{item:summability_L2} follows immediately.
	Regarding \ref{item:summability_H1}, note that the sequence $f^N \coloneqq \sum_{i = 1}^N f_i \varphi_i$ is a Cauchy sequence in $H^1(\Omega)$, since
	\begin{align*}
		\lVert \sum_{i = 1}^N f_i \varphi_i - \sum_{i = 1}^{M-1} f_i \varphi_i \rVert_{H^1(\Omega)}^2
		&= \lVert \sum_{i = M}^N f_i \varphi_i \rVert_{H^1(\Omega)}^2 \\
		&\simeq \lVert \sum_{i = M}^N f_i \varphi_i \rVert_{L^2(\Omega,n)}^2 + \lVert \sum_{i = M}^N f_i \nabla \varphi_i \rVert_{L^2(\Omega)}^2 \\
		&= \sum_{i = M}^N |f_i|^2 + \sum_{i = M}^N |f_i|^2 \lambda_i^2 \rightarrow 0
	\end{align*}
	where we used the orthogonality properties of the eigenfunctions and the assumed convergence of the series.
	We therefore find that
	\begin{equation*}
		\nabla f =  \sum_{i \in \mathbb{N}} f_i \nabla \varphi_i
		\qquad \text{and} \qquad
		\lVert \nabla f \rVert_{L^2(\Omega)}^2 = \sum_{i \in \mathbb{N}} |f_i|^2 \lambda_i^2.
	\end{equation*}
	The estimate for the full $H^1(\Omega)$ norm follows with \ref{item:summability_L2}.
	Interpolation between $L^2(\Omega)$ and $H^1(\Omega)$ gives \eqref{eq:interpolation_L2_H1}.
	The estimate for $f \in L^2_0(\Omega, n)$ follows by norm equivalence.
	For \ref{item:summability_H2}, note that if $\sum_{i \in \mathbb{N}} |f_i|^2 \lambda_i^4 < \infty$ by the above arguments the partial sums $f^N$ converge in $H^1(\Omega)$.
	Furthermore, $f^N$ is a Cauchy sequence in $H^1(\Omega, \Delta) \coloneqq \{ u \in H^1(\Omega) \colon \Delta u \in L^2(\Omega) \}$ equipped with the norm $\lVert u \rVert_{H^1(\Omega)} + \lVert \Delta u \rVert_{L^2(\Omega)}$.
	To show this it suffices to show that $\Delta f^N$ is a Cauchy sequence in $L^2(\Omega)$.
	We have
	\begin{align*}
		\lVert \Delta f^N - \Delta f^{M-1} \rVert_{L^2(\Omega)}^2
		&= \lVert \Delta \sum_{i = 1}^N f_i \varphi_i - \Delta \sum_{i = 1}^{M-1} f_i \varphi_i \rVert_{L^2(\Omega)}^2 \\
		&= \lVert \sum_{i = M}^N f_i \Delta \varphi_i \rVert_{L^2(\Omega)}^2 \\
		&= \lVert \sum_{i = M}^N f_i \lambda_i^2 n^2 \varphi_i \rVert_{L^2(\Omega)}^2 \\
		&\simeq \lVert \sum_{i = M}^N f_i \lambda_i^2 \varphi_i \rVert_{L^2(\Omega, n)}^2 \\
		&= \sum_{i = M}^N |f_i|^2 \lambda_i^4 \rightarrow 0.
	\end{align*}
	Therefore, $f^N$ is a Cauchy sequence in $H^1(\Omega, \Delta)$ and consequently converges.
	Since $\Delta: H^1(\Omega, \Delta) \to L^2(\Omega)$ is continuous, we conclude $\Delta f = \sum_{i \in \mathbb{N}} f_i \Delta \varphi_i = \sum_{i \in \mathbb{N}} f_i \lambda_i^2 n^2 \varphi_i$.
	Furthermore, we have $\partial_n f = 0$.
	This can be easily seen since by the previous arguments $\nabla f \in H(\Omega, \div)$, which gives $\partial_n f = \nabla f \cdot \nu \in H^{-1/2}(\partial \Omega)$.
	Furthermore, we have for any $v \in H^1(\Omega)$
	\begin{equation*}
		\langle \partial_n f, v \rangle
		= (\nabla f, \nabla v) + (\Delta f, v)
		= \lim_{N \to \infty} (\nabla f^N, \nabla v) + (\Delta f^N, v)
		= \lim_{N \to \infty} \langle \underbrace{\partial_n f^N}_{=0}, v \rangle
		= 0
	\end{equation*}
	By elliptic regularity and the assumed regularity of $\partial \Omega$ we find
	\begin{equation*}
		|f|_{H^2(\Omega)}^2 \simeq \lVert \Delta f \rVert_{L^2(\Omega)}^2 = \sum_{i \in \mathbb{N}} |f_i|^2 \lambda_i^4,
	\end{equation*}
	where we again used the orthogonality of the eigenfunctions.
	The remaining estimates follow again by interpolation and norm equivalence.
\end{proof}

\begin{lemma}[Analytic regularity of the eigenfunctions]\label{lemma:analytic_regularity_eigenfunctions}
	Let $\Omega$ be a bounded Lipschitz domain with analytic boundary $\partial \Omega$.
	Let $n$ satisfy Assumption \ref{assumption:general_assumptions}.
	Then there exist constants $C_{\mathrm{eig}}$, $\gamma_{\mathrm{eig}} \geq 0$ independent of $i$ such that
	\begin{itemize}
			\item if $n$ is globally analytic the eigenfunctions are analytic and satisfy
			\begin{equation*}
				\lVert \nabla^p \varphi_i \rVert_{L^2(\Omega)} \leq C_{\mathrm{eig}} \gamma_{\mathrm{eig}}^p \max\{\lambda_i, p\}^p , \qquad \forall p \in \mathbb{N}_0.
			\end{equation*}
			\item if $n$ is piecewise analytic with analytic interface $\Gamma_i$ the eigenfunctions are piecewise analytic and  satisfy
			\begin{equation*}
				\lVert \nabla^p \varphi_i \rVert_{L^2(\Omega \setminus \Gamma_i)} \leq C_{\mathrm{eig}} \gamma_{\mathrm{eig}}^p \max\{\lambda_i, p\}^p, \qquad \forall p \in \mathbb{N}_0.
			\end{equation*}
	\end{itemize}
\end{lemma}

\begin{proof}
	The proof follows closely the reasoning in \cite[Lemma C.1]{melenk12}.
	For the readers convenience we repeat certain arguments.
	We will employ \cite[Prop. 5.5.1]{melenk02} (interior analytic regularity) and \cite[Prop. 5.5.3]{melenk02} (boundary analytic regularity for Neumann problems)
	in the globally analytic case
	as well as \cite[Prop. 5.5.4]{melenk02} (interface analytic regularity) in the piecewise analytic case.
	The argument is a local one, i.e., the domain, the boundary and the interface are covered by a finite number of balls and the above Propositions are applied.
	We will only present the application of \cite[Prop. 5.5.1]{melenk02}, i.e., interior regularity.
	To that end we rewrite the eigenvalue problem \eqref{eq:heterogeneuos_eigenvalue_problem} as
	\begin{equation}
		\begin{alignedat}{2}
			  - \lambda_i^{-2} \Delta \varphi_i  - n^2 \varphi_i  &= 0 \quad   &&\text{in } \Omega,\\
		   \lambda_i^{-2} \partial_n \varphi_i &= 0                          &&\text{on } \partial \Omega.
		\end{alignedat}
	\end{equation}
	Regarding interior regularity, fix an open subset $U \subset \Omega$, such that the closure $\overline{U}$ is completely contained in $\Omega$.
	With an appropriate change of variables and the choices $\varepsilon = \lambda_i^{-1}$, $C_A = 1$, $\gamma_A = 0$, $C_b = 0$, $\gamma_b = 0$, $C_c = C_n$, $\gamma_c = \gamma_n$, $C_f = 0$ and $\gamma_f = 0$
	we apply \cite[Prop. 5.5.1]{melenk02} which gives
	\begin{equation*}
		\lVert \nabla^{p+2} \varphi_i \rVert_{L^2(U)} \leq C K^{p+2} \max\{p+2, \lambda_i\}^{p+2}(\lambda_i^{-1} \lVert \nabla \varphi_i \rVert_{L^2(\Omega)} + \lVert \varphi_i \rVert_{L^2(\Omega)}).
	\end{equation*}
	Combined with the fact $\lVert \nabla \varphi_i \rVert_{L^2(\Omega)} = \lambda_i$ and $\lVert \varphi_i \rVert_{L^2(\Omega)} = 1$, due to Theorem \ref{theorem:results_on_eigenfunctions}, we find
	\begin{equation*}
		\lVert \nabla^{p} \varphi_i \rVert_{L^2(U)} \leq C K^{p} \max\{\lambda_i, p\}^{p}.
	\end{equation*}
	Nearly analogous arguments can be repeated for the boundary and the interface using \cite[Prop. 5.5.3]{melenk02} and \cite[Prop. 5.5.4]{melenk02} respectively.
	Covering $\Omega$, the boundary $\partial \Omega$ and the interface $\Gamma_i$ with a finite number of open balls then yields the result.
\end{proof}

\begin{remark}
	The constants $C_{\mathrm{eig}}$ and $\gamma_{\mathrm{eig}}$ in Lemma \ref{lemma:analytic_regularity_eigenfunctions} depend on $C_n$ and $\gamma_n$.
\end{remark}

We introduce the appropriate high and low pass filters in a heterogeneous setting.
For $\eta > 1$ we define the operators $\lowPassFilter \colon L^2(\Omega) \rightarrow L^2(\Omega)$ and $\highPassFilter \colon L^2(\Omega) \rightarrow L^2(\Omega)$ via
\begin{equation*}
  \lowPassFilter f = \sum_{i \in \mathbb{N} \colon \lambda_i < \eta k} f_i \varphi_i, \qquad \highPassFilter f = \sum_{i \in \mathbb{N} \colon \lambda_i \geq \eta k} f_i \varphi_i, \qquad f = \sum_{i \in \mathbb{N}} f_i \varphi_i,
\end{equation*}
see also \cite[Section 4]{melenk-sauter11} for the analogous operators in a homogeneous setting.
We collect some immediate results concerning these operators in the following
\begin{lemma}[Properties of $\lowPassFilter$ and $\highPassFilter$]\label{lemma:elementary_properties_high_low_pass_filter}
  The operators $\lowPassFilter$ and $\highPassFilter$ are bounded, linear and satisfy $\lowPassFilter f + \highPassFilter f = f$.
	Furthermore, $\highPassFilter f \in L^2_0(\Omega, n)$.
	Finally, there holds
	\begin{align*}
	  \lVert \lowPassFilter f \rVert_{L^2(\Omega, n)}^2 &= \sum_{i \in \mathbb{N} \colon \lambda_i < \eta k} |f_i|^2 \leq \lVert f \rVert_{L^2(\Omega, n)}^2, \\
	  \lVert \highPassFilter f \rVert_{L^2(\Omega, n)}^2 &= \sum_{i \in \mathbb{N} \colon \lambda_i \geq \eta k} |f_i|^2 \leq \lVert f \rVert_{L^2(\Omega, n)}^2.
	\end{align*}
\end{lemma}
\begin{proof}
	To see that $\highPassFilter f \in L^2_0(\Omega, n)$ just note that the eigenfunction corresponding to the zero eigenvalue is not part of the summation.
	The rest is obvious.
\end{proof}

\begin{lemma}[Analytic regularity of $\lowPassFilter f$]\label{lemma:analytic_regularity_lowpassfilter}
	Let $\Omega$ be a bounded Lipschitz domain with analytic boundary $\partial \Omega$.
	Let $n$ satisfy Assumption \ref{assumption:general_assumptions}.
	Then there exist constants $C_{L}$, $\gamma_{L} \geq 0$ such that
	\begin{itemize}
			\item if $n$ is globally analytic the low frequency part $\lowPassFilter f$ is analytic and satisfy
			\begin{equation*}
				\lVert \nabla^p \lowPassFilter f \rVert_{L^2(\Omega)}	\leq C_L \gamma_{L}^p \max\{\eta k, p\}^p  \lVert f \rVert_{L^2(\Omega)} , \qquad \forall p \in \mathbb{N}_0.
			\end{equation*}
			\item if $n$ is piecewise analytic the low frequency part $\lowPassFilter f$ is piecewise analytic and satisfy
			\begin{equation*}
				\lVert \nabla^p \lowPassFilter f \rVert_{L^2(\Omega \setminus \Gamma_i)}	\leq C_L \gamma_{L}^p \max\{\eta k, p\}^p  \lVert f \rVert_{L^2(\Omega)} , \qquad \forall p \in \mathbb{N}_0.
			\end{equation*}
	\end{itemize}
\end{lemma}
\begin{proof}
	The (piecewise) analyticity is obvious since $\lowPassFilter f$ is the finite sum of (piecewise) analytic functions, see Lemma \ref{lemma:analytic_regularity_eigenfunctions}.
	With Lemma \ref{lemma:analytic_regularity_eigenfunctions} we estimate
	\begin{align*}
		\lVert \nabla^p \lowPassFilter f \rVert_{L^2(\Omega)}
		&= \left \lVert \sum_{i \in \mathbb{N} \colon \lambda_i < \eta k} f_i  \nabla^p \varphi_i \right\rVert_{L^2(\Omega)} \\
		&\leq \sum_{i \in \mathbb{N} \colon \lambda_i < \eta k} | f_i | \lVert \nabla^p \varphi_i \rVert_{L^2(\Omega)} \\
		&\leq \sum_{i \in \mathbb{N} \colon \lambda_i < \eta k} | f_i |  C_{\mathrm{eig}} \gamma_{\mathrm{eig}}^p \max\{\lambda_i, p\}^p \\
		&\leq C_{\mathrm{eig}} \gamma_{\mathrm{eig}}^p \max\{\eta k, p\}^p \sum_{i \in \mathbb{N} \colon \lambda_i < \eta k} | f_i |.
	\end{align*}
	Using the Cauchy-Schwarz inequality we find
	\begin{equation*}
		\sum_{i \in \mathbb{N} \colon \lambda_i \leq \eta k} | f_i |
		\leq \sqrt{\sum_{i \in \mathbb{N} \colon \lambda_i < \eta k}  1 } \cdot \sqrt{\sum_{i \in \mathbb{N} \colon \lambda_i < \eta k} | f_i |^2}
		\lesssim \sqrt{ \# \{i \in \mathbb{N} \colon \lambda_i < \eta k \} } \cdot \lVert f \rVert_{L^2(\Omega)}.
	\end{equation*}
	Due to norm equivalence between $L^2(\Omega)$ and $L^2(\Omega, n)$ together with the representation of eigenvalues via the Rayleigh quotient we find that $\lambda_i$ behave like standard eigenvalues of the Laplacian.
 	Finally, due to Weyl's law, we find
	\TODO{reference for weyls law}
	\begin{equation*}
		\# \{i \in \mathbb{N} \colon \lambda_i < \eta k \} \simeq (\eta k)^d
	\end{equation*}
	Putting everything together we find
	\begin{equation*}
		\lVert \nabla^p \lowPassFilter f \rVert_{L^2(\Omega)}
		\leq C_L \gamma_{L}^p \max\{\eta k, p\}^p (\eta k)^{d/4}  \lVert f \rVert_{L^2(\Omega)}
		\leq C_L \gamma_{L}^p \max\{\eta k, p\}^p  \lVert f \rVert_{L^2(\Omega)}.
	\end{equation*}
	For piecewise analytic $n$ the proof is analogous.
\end{proof}

In the following we analyze the mapping properties of certain solution operators, which will be used in Lemma \ref{lemma:contraction_argument}, the contraction argument, later on.
\begin{itemize}
	\item \textbf{The Operator $S_k$}: Let $S_k: L^2(\Omega) \rightarrow H^1(\Omega)$ denote the solution operator mapping $f \in L^2(\Omega)$ to $S_k(f) \coloneqq u$, where $u \in H^1(\Omega)$ is the weak solution of
	\begin{equation}
		\begin{alignedat}{2}
			- \Delta u - k^2 n^2 u &= n^2 f \quad   &&\text{in } \Omega,\\
			\partial_n u - i k u   &= 0             &&\text{on } \partial \Omega.
		\end{alignedat}
	\end{equation}
	\item \textbf{The Operator $N_k$}: For $k^2 \notin \{ \lambda_i^2 \}_{i \in \mathbb{N}}$ let $N_k: L^2_0(\Omega, n) \rightarrow H^1(\Omega)$ be given by the representation formula
	\begin{equation}\label{eq:operator_N_representation_formula}
		N_k(f) \coloneqq \sum_{i \in \mathbb{N}} \frac{1}{\lambda_i^2 - k^2} f_i \varphi_i.
	\end{equation}
	We summarize properties of $N_k$ in Lemma \ref{lemma:mapping_properties_N}.
	\item \textbf{The Operator $S_k^+$}: Let $S_k^+: L^2(\partial \Omega) \rightarrow H^1(\Omega)$ denote the solution operator mapping $g \in L^2(\partial \Omega)$ to $S_k^+(g) \coloneqq w$, where $w \in H^1(\Omega)$ is the weak solution of
	\begin{equation}\label{eq:heterogeneous_good_helmholtz}
		\begin{alignedat}{2}
			- \Delta w + k^2 n^2 w &= 0     \quad   &&\text{in } \Omega,\\
			\partial_n w - i k w   &= g             &&\text{on } \partial \Omega.
		\end{alignedat}
	\end{equation}
	We summarize properties of $S_k^+$ in Lemma \ref{lemma:mapping_properties_heterogeneous_good_helmholtz}.
\end{itemize}

We remind the reader the multiplicative trace inequality.

\begin{proposition}[{\cite[Thm. A.2]{melenk05}}]\label{proposition:multiplicative_trace_inquality}
	Let $ \Omega \subset \mathbb{R}^d $ be a Lipschitz domain and $ s \in ( 1/2, 1 ] $.
	Then there exists a constant $ C > 0 $ such that for all $ u \in H^s(\Omega) $ there holds
	\begin{equation*}
		\lVert u \rVert_{L^2(\partial \Omega)}
			\leq C
			\lVert u \rVert_{L^2(\Omega)}^{1-1/(2s)}
			\lVert u \rVert_{H^s(\Omega)}^{1/(2s)},
	\end{equation*}
	where the left-hand side is understood in the trace sense.
\end{proposition}

\begin{lemma}[Mapping properties of $N_k$ and $N_k \circ \highPassFilter$]\label{lemma:mapping_properties_N}
	Let $\Omega$ be a bounded Lipschitz domain.
	For $k^2 \notin \{ \lambda_i^2 \}_{i \in \mathbb{N}}$
	the operator $N_k$ given by \eqref{eq:operator_N_representation_formula} for $f \in L^2_0(\Omega, n)$ maps in fact into $H^1(\Omega) \cap L^2_0(\Omega, n)$.
	The function $v \coloneqq N_k(f)$ solves
	\begin{equation}\label{eq:operator_N_pde}
		\begin{alignedat}{2}
			- \Delta v - k^2 n^2 v &= n^2 f \quad   &&\text{in } \Omega,\\
								\partial_n v &= 0             &&\text{on } \partial \Omega.
		\end{alignedat}
	\end{equation}
	Furthermore, the composition $N_k \circ \highPassFilter \colon L^2(\Omega) \to H^1(\Omega)$ is well defined for every $k \geq k_0 > 0$.
	Additionally the estimates
	\begin{align*}
		\lVert N_k( \highPassFilter f )\rVert_{L^2(\Omega)} &\lesssim (\eta k)^{-2} \lVert f \rVert_{L^2(\Omega)} \\
		\lVert N_k( \highPassFilter f )\rVert_{H^1(\Omega)} &\lesssim (\eta k)^{-1} \lVert f \rVert_{L^2(\Omega)}
	\end{align*}
	hold.
	Finally, if $\partial \Omega$ is $C^2$ or $\Omega$ is a convex polygon the estimate
	\begin{equation*}
		\lVert N_k( \highPassFilter f )\rVert_{H^2(\Omega)} \lesssim \lVert f \rVert_{L^2(\Omega)}
	\end{equation*}
	holds.
\end{lemma}

\begin{proof}
	The fact that $N_k(f) \in L^2_0(\Omega, n)$ for $f \in L^2_0(\Omega, n)$ is obvious since by definition the Fourier coefficient of $N_k(f)$ corresponding to the zero eigenvalue is also zero.
	To see $N_k(f) \in H^1(\Omega)$, we employ Lemma \ref{lemma:connection_summability_regularity}, which is applicable since
	\begin{equation*}
		\sum_{i \in \mathbb{N}} \left(\frac{1}{\lambda_i^2 - k^2} |f_i| \right)^2 \lambda_i^2 < \infty.
	\end{equation*}
	To verify that $N_k(f)$ solves \eqref{eq:operator_N_pde} it suffices to calculate the Fourier coefficient of a weak solution to problem \eqref{eq:operator_N_pde}.
	Let $v \in H^1(\Omega) \cap L^2_0(\Omega, n)$ be a weak solution to problem \eqref{eq:operator_N_pde}.
	Again denote by $v_i$ the corresponding Fourier coefficients.
	Testing the equation with $\varphi_i$ and using the equation satisfied by $\varphi_i$ we find
	\begin{equation*}
		\underbrace{(\nabla v, \nabla \varphi_i)}_{=\lambda_i^2 (v, \varphi_i)_{L^2(\Omega, n)}} - k^2 \underbrace{(v, \varphi_i)_{L^2(\Omega, n)}}_{=v_i} = \underbrace{(f, \varphi_i)_{L^2(\Omega, n)}}_{=f_i}
	\end{equation*}
	Therefore, the Fourier coefficients $v_i$ are given by $v_i = 1/(\lambda_i^2 - k^2) f_i$.
	A density argument for the eigenfunctions then yields the result.
	Since the high pass filter $\highPassFilter$ just sets certain Fourier coefficients to zero we immediately have for $f \in L^2(\Omega)$
	\begin{equation*}
		N_k( \highPassFilter f ) = \sum_{i \in \mathbb{N} \colon \lambda_i \geq \eta k} \frac{1}{\lambda_i^2 - k^2} f_i \varphi_i.
	\end{equation*}
	Since $\eta > 1$ this sum is always well defined.
	Regarding the norm estimates we again employ Lemma \ref{lemma:connection_summability_regularity}.
	We estimate
	\begin{align*}
		\lVert N_k( \highPassFilter f )\rVert_{L^2(\Omega)}^2
		&\simeq \lVert N_k( \highPassFilter f )\rVert_{L^2(\Omega, n)}^2 \\
		&= \sum_{i \in \mathbb{N} \colon \lambda_i \geq \eta k} \left( \frac{1}{\lambda_i^2 - k^2} |f_i| \right)^2 \\
		&\lesssim (\eta k)^{-4} \sum_{i \in \mathbb{N} \colon \lambda_i \geq \eta k} |f_i|^2 \\
		&\lesssim (\eta k)^{-4} \lVert f \rVert_{L^2(\Omega)}^2.
	\end{align*}
	The other estimates follow by similar calculations.
\end{proof}

\begin{lemma}[Mapping properties of $ S_k^+ $]\label{lemma:mapping_properties_heterogeneous_good_helmholtz}
	Let $\Omega$ be a bounded Lipschitz domain.
	For $g \in L^2(\partial \Omega)$ the solution operator $S_k^+(g) \coloneqq w$ of problem \eqref{eq:heterogeneous_good_helmholtz} satisfies
	\begin{align}
		\lVert w \rVert_{L^2(\partial \Omega)} &\lesssim k^{-1} \lVert g \rVert_{L^2(\partial \Omega)},                            \label{eq:good_helmholtz_trace_estimate}  \\
		\lVert w \rVert_{H^1(\Omega)} + k \lVert w \rVert_{L^2(\Omega)} &\lesssim k^{-1/2} \lVert g \rVert_{L^2(\partial \Omega)}. \label{eq:good_helmholtz_volume_estimate}
	\end{align}
	Furthermore, if $\partial \Omega$ is smooth and $g \in H^{1/2}(\partial \Omega)$ or if $\Omega$ is a convex polygon in 2D and $g \in H^{1/2}_{pw}(\partial \Omega)$ the the solutions $w$ satisfies $w \in H^2(\Omega)$ as well as
	\begin{equation}\label{eq:good_helmholtz_H2_estimate}
		\lVert w \rVert_{H^2(\Omega)} \lesssim \lVert g \rVert_{H^{1/2}(\partial \Omega)} + k^{1/2} \lVert g \rVert_{L^2(\partial \Omega)}.
	\end{equation}
	All hidden constants are independent of $k$.
\end{lemma}

\begin{proof}
	The solution $w$ satisfies the weak formulation
	\begin{equation*}
		(\nabla w, \nabla z) + k^2 (w, z)_{L^2(\Omega, n)} - ik \langle w, z \rangle = \langle g, z \rangle \qquad \forall z \in H^1(\Omega).
	\end{equation*}
	Choosing $z=w$, taking the imaginary part and applying the Cauchy-Schwarz inequality immediately gives the estimate \eqref{eq:good_helmholtz_trace_estimate}.
	Taking the real part, applying the Cauchy-Schwarz inequality, using the previous estimate as well as norm equivalence between $L^2(\Omega)$ and $L^2(\Omega, n)$ gives estimate \eqref{eq:good_helmholtz_volume_estimate}.
	Regarding the regularity shift, note that $w$ satisfies the Neumann problem
	\begin{equation}
		\begin{alignedat}{2}
			- \Delta w   &= - k^2 n^2 w      \quad   &&\text{in } \Omega,\\
			\partial_n w &= g + i k w                &&\text{on } \partial \Omega.
		\end{alignedat}
	\end{equation}
	Consequently $w \in H^2(\Omega)$ with the estimate
	\begin{align*}
		\lVert w \rVert_{H^2(\Omega)}
		&\lesssim \lVert - k^2 n^2 w \rVert_{L^2(\Omega)} + \lVert g + i k w \rVert_{H^{1/2}(\partial \Omega)} \\
		&\lesssim k^2 \lVert w \rVert_{L^2(\Omega)} + \lVert g \rVert_{H^{1/2}(\partial \Omega)} + k \rVert w \rVert_{H^{1/2}(\partial \Omega)} \\
		&\lesssim k^2 \lVert w \rVert_{L^2(\Omega)} + k \rVert w \rVert_{H^{1}(\Omega)} + \lVert g \rVert_{H^{1/2}(\partial \Omega)}.
	\end{align*}
	Estimate \eqref{eq:good_helmholtz_volume_estimate} then yields the result.
\end{proof}

\begin{remark}
	Before turning to the contraction argument in Lemma \ref{lemma:contraction_argument} there are a few remarks to be made.
	\begin{itemize}
		\item For the splitting made in Lemma \ref{lemma:contraction_argument} it is important to note that the smoothness assumption on $n$ solely enters in the analytic part.
		\item The eigenfunction expansion, the mapping properties of the above solution operators, especially all the $H^2(\Omega)$ estimates work out with the minimal assumption of $n$ being uniformly bounded on $\overline{\Omega}$.
	\end{itemize}
\end{remark}

\begin{lemma}[Analytic regularity of $S_k(\lowPassFilter f)$]\label{lemma:analytic_regularity_solution_for_lowpassfilter}
	Let Assumption \ref{assumption:general_assumptions} be valid.
	Then there exist constants $C_A$, $\gamma_A \geq 0$ independent of $k$, such that for every $f \in L^2(\Omega)$,
	the function $u_A \coloneqq S_k(\lowPassFilter f)$ is (piecewise) analytic if $n$ is (piecewise) analytic, and satisfies
	\begin{equation}\label{eq:u_analytic_energy_norm_estimate}
		\lVert \nabla u_A \rVert_{L^2(\Omega)} + k \lVert u_A \rVert_{L^2(\Omega)} \leq C_A \StabilityConstant \lVert f \rVert_{L^2(\Omega)}.
	\end{equation}
	If $n$ is globally analytic we additionally have
	\begin{equation}\label{eq:u_analytic_estimate_global}
		\lVert \nabla^p u_A \rVert_{L^2(\Omega)}	 \leq C_A \gamma_{A}^p \max\{\eta k, p\}^p  \StabilityConstant k^{-1} \lVert f \rVert_{L^2(\Omega)} , \qquad \forall p \geq 2.
	\end{equation}
	In the case of piecewise analytic $n$ we have
	\begin{equation}\label{eq:u_analytic_estimate_piecewise}
		\lVert \nabla^p u_A \rVert_{L^2(\Omega \setminus \Gamma_i)}	\leq C_A \gamma_{A}^p \max\{\eta k, p\}^p  \StabilityConstant k^{-1} \lVert f \rVert_{L^2(\Omega)} , \qquad \forall p \geq 2.
	\end{equation}
\end{lemma}

\begin{proof}
	Estimate \eqref{eq:u_analytic_energy_norm_estimate} follows by the stability estimate \eqref{eq:stability_estimate}
	in Assumption \ref{assumption:general_assumptions} together with the estimate for the low pass filter in Lemma \ref{lemma:elementary_properties_high_low_pass_filter}:
	\begin{equation*}
		\lVert \nabla u_A \rVert_{L^2(\Omega)} + k \lVert \nabla u_A \rVert_{L^2(\Omega)}
		\leq \StabilityConstant \lVert n^2 \lowPassFilter f \rVert_{L^2(\Omega)}
		\lesssim \StabilityConstant \lVert f \rVert_{L^2(\Omega)}.
	\end{equation*}
	We turn towards estimate \eqref{eq:u_analytic_estimate_global}.
	Estimate  \eqref{eq:u_analytic_estimate_piecewise} follows analogously.
	To that end, note that $u_A$ solves \eqref{eq:heterogeneous_helmholtz_boundary_value_problem_new} with right hand side $n^2 \lowPassFilter f$,
	which is the product of two analytic functions, i.e., $n^2$, which is analytic by assumption, and $\lowPassFilter f$, which is analytic due to Lemma \ref{lemma:analytic_regularity_lowpassfilter}.
	Therefore \cite[Lemma 4.3.1]{melenk02} is applicable, and consequently the right hand side is again analytic with corresponding estimates.
	Finally, as in the proof of Lemma \ref{lemma:analytic_regularity_eigenfunctions},
	we apply \cite[Prop. 5.5.1]{melenk02} (interior analytic regularity) and \cite[Prop. 5.5.3]{melenk02} (boundary analytic regularity for Neumann problems)
	in the globally analytic case as well as \cite[Prop. 5.5.4]{melenk02} (interface analytic regularity) in the piecewise analytic case,
	to a rescaled version of problem \eqref{eq:heterogeneous_helmholtz_boundary_value_problem_new}.
	Via the scaling $\varepsilon \coloneqq 1/k$ the function $u_A$ satisfies
	\begin{equation*}
		\begin{alignedat}{2}
			- \varepsilon^2 \Delta u_A - n^2 u_A &= \varepsilon^2 n^2 \lowPassFilter f \quad   &&\text{in } \Omega,\\
			\varepsilon^2 \partial_n u_A &= \varepsilon i u_A    															&&\text{on } \partial \Omega.
		\end{alignedat}
	\end{equation*}
	from now on the proof is as in Lemma \ref{lemma:analytic_regularity_eigenfunctions}.
	We therefore arrive at
	\begin{equation}
		\lVert \nabla^p u_A \rVert_{L^2(\Omega)}	 \lesssim C_A \gamma_{A}^p \max\{\eta k, p\}^p  ( k^{-2} \lVert f \rVert_{L^2(\Omega)} + k^{-1} \lVert \nabla u_A \rVert_{L^2(\Omega)} +  \lVert u_A \rVert_{L^2(\Omega)}), \qquad \forall p \geq 2.
	\end{equation}
	Finally applying estimate \eqref{eq:u_analytic_energy_norm_estimate} yields the result.
	See also \cite[Lemma 4.12]{melenk-sauter11} for similar arguments in the homogeneous case.
\end{proof}

\begin{lemma}[Contraction argument]\label{lemma:contraction_argument}
	Let Assumption \ref{assumption:general_assumptions} be valid.
	Let $q \in (0, 1)$ be given.
	Then there exist constants $C$, $\gamma \geq 0$ independent of $k$ such that for every $f \in L^2(\Omega)$ the function $u = S_k(f)$ can be written as $u = u_{H^2} + u_A + S_k(\tilde{f})$, where
	\begin{align}
		\lVert u_{H^2} \rVert_{H^2(\Omega)} + k\lVert u_{H^2} \rVert_{H^1(\Omega)} + k^2 \lVert u_{H^2} \rVert_{L^2(\Omega)} &\leq C \lVert f \rVert_{L^2(\Omega)}, \\
		\lVert \nabla u_A \rVert_{L^2(\Omega)} + k \lVert u_A \rVert_{L^2(\Omega)} &\leq C \StabilityConstant \lVert f \rVert_{L^2(\Omega)}.
	\end{align}
	If $n$ is globally analytic we additionally have
	\begin{equation*}
		\lVert \nabla^p u_A \rVert_{L^2(\Omega)} \leq C \gamma^p \max\{k, p\}^p  \StabilityConstant k^{-1} \lVert f \rVert_{L^2(\Omega)} , \qquad \forall p \geq 2.
	\end{equation*}
	In the case of piecewise analytic $n$ we have
	\begin{equation*}
		\lVert \nabla^p u_A \rVert_{L^2(\Omega \setminus \Gamma_i)} \leq C \gamma^p \max\{k, p\}^p  \StabilityConstant k^{-1} \lVert f \rVert_{L^2(\Omega)} , \qquad \forall p \geq 2.
	\end{equation*}
	Finally, the data $\tilde{f}$ contracts, i.e.,
	\begin{equation*}
		\lVert \tilde{f} \rVert_{L^2(\Omega)} \leq q \lVert f \rVert_{L^2(\Omega)}.
	\end{equation*}
\end{lemma}

\begin{proof}
	We split the solution $u$ as follows
	\begin{equation*}
		S_k(f) = u = \underbrace{N_k(\highPassFilter f)}_{\eqqcolon u_{H^2, I}} + \underbrace{S_k(\lowPassFilter f)}_{\eqqcolon u_A} + r,
	\end{equation*}
	where $r$ satisfies
	\begin{equation}
		\begin{alignedat}{2}
			- \Delta r - k^2 n^2 r &= 0                \quad       &&\text{in } \Omega,\\
			\partial_n u - i k u   &= i k u_{H^2, I}      \quad       &&\text{on } \partial \Omega.
		\end{alignedat}
	\end{equation}
	The function $r$ is split into
	\begin{equation*}
		r = S_k^+(i k u_{H^2, I}) + \tilde{r}
	\end{equation*}
	where $\tilde{r}$ satisfies
	\begin{equation}
		\begin{alignedat}{2}
			- \Delta \tilde{r} - k^2 n^2 \tilde{r} &= 2 k^2 n^2 S_k^+(i k u_{H^2, I}) \quad   &&\text{in } \Omega,\\
			\partial_n \tilde{r} - i k \tilde{r}   &= 0                                    &&\text{on } \partial \Omega.
		\end{alignedat}
	\end{equation}
	Summarizing we have
	\begin{equation*}
		S_k(f) = u = u_{H^2} + u_A + S_k(\tilde{f})
	\end{equation*}
	with
	\begin{equation*}
		 u_{H^2} \coloneqq u_{H^2, I} + S_k^+(i k u_{H^2, I}), \qquad u_A \coloneqq S_k(\lowPassFilter f), \qquad \tilde{f} \coloneqq 2 k^2 n^2 S_k^+(i k u_{H^2, I}).
	\end{equation*}
	At this point the parameter $\eta$ in the definition of the low and high pass filters is still at our disposal and will be selected at the end of the proof.
	By Lemma \ref{lemma:mapping_properties_N} since $u_{H^2, I} = N_k(\highPassFilter f)$ we find
	\begin{equation}\label{eq:estimate_u_H2_I}
		\lVert u_{H^2, I} \rVert_{H^2(\Omega)} + \eta k \lVert u_{H^2, I} \rVert_{H^1(\Omega)} + (\eta k)^2 \lVert u_{H^2, I} \rVert_{L^2(\Omega)}
		\lesssim \lVert f \rVert_{L^2(\Omega)}.
	\end{equation}
	Applying Lemma \ref{lemma:mapping_properties_heterogeneous_good_helmholtz},
	using the multiplicative trace inequality for $s = 1$ given in Proposition \ref{proposition:multiplicative_trace_inquality}
	and the estimate \eqref{eq:estimate_u_H2_I} we find
	\begin{equation}\label{eq:estimate_u_H2_second_part}
		\begin{alignedat}{3}
		\lVert S_k^+(i k u_{H^2, I}) \rVert_{H^2(\Omega)} &+ k \lVert S_k^+(i k u_{H^2, I}) \rVert_{H^1(\Omega)} + k^2 \lVert S_k^+(i k u_{H^2, I}) \rVert_{L^2(\Omega)} \\
		&\lesssim \lVert i k u_{H^2, I} \rVert_{H^{1/2}(\partial \Omega)} + k^{1/2} \lVert i k u_{H^2, I} \rVert_{L^2(\partial \Omega)} \\
		&\lesssim k \lVert u_{H^2, I} \rVert_{H^{1}(\Omega)} + k^{3/2} \lVert u_{H^2, I} \rVert_{L^2(\Omega)}^{1/2} \lVert u_{H^2, I} \rVert_{H^1(\Omega)}^{1/2} \\
		&\lesssim \eta^{-1} \lVert f \rVert_{L^2(\Omega)},
		\end{alignedat}
	\end{equation}
	which gives the estimate for $u_{H^2}$.
	The estimates for $u_A$ follow immediately by Lemma \ref{lemma:analytic_regularity_solution_for_lowpassfilter}.
	We estimate $\lVert \tilde{f} \rVert_{L^2(\Omega)}$ using the above estimate \eqref{eq:estimate_u_H2_second_part} as follows
	\begin{equation*}
		\lVert \tilde{f} \rVert_{L^2(\Omega)}
		= \lVert 2 k^2 n^2 S_k^+(i k u_{H^2, I})\rVert_{L^2(\Omega)} \\
		\lesssim k^2 \lVert S_k^+(i k u_{H^2, I})\rVert_{L^2(\Omega)} \\
		\leq C_0 \eta^{-1} \lVert f \rVert_{L^2(\Omega)},
	\end{equation*}
	for some wavenumber independent constant $C_0>1$.
	We fix $\eta > 1$ such that $C_0 \eta^{-1} = q$, which concludes the proof.
\end{proof}

The contraction argument in Lemma \ref{lemma:contraction_argument} enables us to prove the existence of the following decomposition.
\begin{theorem}[Iteration argument]\label{theorem:iteration_argument}
	Let Assumption \ref{assumption:general_assumptions} be valid.
	Then there exist constants $C$, $\gamma \geq 0$ independent of $k$ such that for every $f \in L^2(\Omega)$ the function $u = S_k(f)$ can be written as $u = u_{H^2} + u_A$, where
	\begin{align*}
		\lVert u_{H^2} \rVert_{H^2(\Omega)} + k\lVert u_{H^2} \rVert_{H^1(\Omega)} + k^2 \lVert u_{H^2} \rVert_{L^2(\Omega)} &\leq C \lVert f \rVert_{L^2(\Omega)}, \\
		\lVert \nabla u_A \rVert_{L^2(\Omega)} + k \lVert u_A \rVert_{L^2(\Omega)} &\leq C \StabilityConstant \lVert f \rVert_{L^2(\Omega)}.
	\end{align*}
	If $n$ is globally analytic we additionally have
	\begin{equation*}
		\lVert \nabla^p u_A \rVert_{L^2(\Omega)} \leq C \gamma^p \max\{k, p\}^p  \StabilityConstant k^{-1} \lVert f \rVert_{L^2(\Omega)} , \qquad \forall p \geq 2.
	\end{equation*}
	In the case of piecewise analytic $n$ we have
	\begin{equation*}
		\lVert \nabla^p u_A \rVert_{L^2(\Omega \setminus \Gamma_i)} \leq C \gamma^p \max\{k, p\}^p  \StabilityConstant k^{-1} \lVert f \rVert_{L^2(\Omega)} , \qquad \forall p \geq 2.
	\end{equation*}
\end{theorem}

\begin{proof}
	The proof iterates the contraction argument in Lemma \ref{lemma:contraction_argument}.
	To that end let $f^{(0)} \coloneqq f$.
	By Lemma \ref{lemma:contraction_argument} we can split $S_k(f^{(0)})$ as follows
	\begin{equation*}
		S_k(f^{(0)}) = u_{H^2}^{(0)} + u_A^{(0)} + S_k(f^{(1)}),
	\end{equation*}
	with $\lVert f^{(1)} \rVert_{L^2(\Omega)} \leq q \lVert f^{(0)} \rVert_{L^2(\Omega)}$.
	We iteratively define the function sequences $u_{H^2}^{(i)}$, $u_A^{(i)}$ and $f^{(i)}$ for $i \in \mathbb{N}$.
	Due to the contraction argument we have $\lVert f^{(i)} \rVert_{L^2(\Omega)} \leq q^i \lVert f \rVert_{L^2(\Omega)}$ and therefore find
	\begin{equation*}
		u = \underbrace{\sum_{i \in \mathbb{N}_0} u_{H^2}^{(i)}}_{\eqqcolon u_{H^2}} + \underbrace{\sum_{i \in \mathbb{N}_0} u_{A}^{(i)}}_{\eqqcolon u_{A}},
	\end{equation*}
	with $u_{H^2}$ and $u_{A}$ being well defined and satisfying the asserted estimates due to a geometric series argument.
	We showcase this argument for the $H^2(\Omega)$ norm of $u_{H^2}$:
	\begin{equation*}
		\lVert u_{H^2} \rVert_{H^2(\Omega)}
		\leq \sum_{i \in \mathbb{N}_0} \lVert u_{H^2}^{(i)} \rVert_{H^2(\Omega)}
		\lesssim \sum_{i \in \mathbb{N}_0} \lVert f^{(i)} \rVert_{L^2(\Omega)}
		\leq \sum_{i \in \mathbb{N}_0} q^i \lVert f \rVert_{L^2(\Omega)}
		\leq C \lVert f \rVert_{L^2(\Omega)}.
	\end{equation*}
	The other estimates follow analogously.
\end{proof}


==> 00_overview_table.tex <==
% !TEX root = main.tex
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Model                   &  Energy Space                                   & $\Lkm$                                                                   & $\Lkp$                                                               & $ \TkOmegaM - \TkOmegaP $               & $\TkGammaM$                             & $\TkGammaP$              & $ \TkGammaM - \TkGammaP $ \\ \hline
HH + Robin BC (Sec.~\ref{problem:HH_with_robin_bc})                & \multirow{5}{*}{$H^1(\Omega)$}                  & \multirow{3}{*}{$-\nabla \cdot (A \nabla u) - k^2 n^2 u$}                & \multirow{4}{*}{$-\nabla \cdot (A \nabla u) + k^2 u$}                & \multirow{3}{*}{$k^2(n^2+1)u$}         & $iku$                                   & $0$                      & $iku$                     \\ \cline{1-1} \cline{6-8}
HH + DtN Sphere (Sec.~\ref{problem:HH_full_space})        &                                                 &                                                                          &                                                                      &                                         & $\mathrm{DtN}_k$                        & $\mathrm{DtN}_0$         & $k R_\Gamma$              \\ \cline{1-1} \cline{6-8}
HH + DtN $\Gamma$ (Sec.~\ref{problem:HH_full_space})       &                                                 &                                                                          &                                                                      &                                         & $\mathrm{DtN}_k$                        & $\mathrm{DtN}_0$         & $k R_\Gamma + A_\Gamma$   \\ \cline{1-1} \cline{3-3} \cline{5-8}
HH + Damping + Robin BC (Sec.~\ref{problem:HH_with_robin_bc})     &                                                 & $-\nabla \cdot (A \nabla u) - k^2 n^2 u + ikmu$                          &                                                                      & $k^2(n^2+1)u - ikmu$                   & $iku$                                   & $0$                      & $iku$                     \\ \cline{1-1} \cline{3-8}
%HH + PML + Robin BC (Sec.~\ref{problem:PML})         &                                                 & $-\nabla(A^{PML}_k \nabla u) - k^2 n^2 u$                                & $-\nabla(A^{PML}_k \nabla u) + k^2 u$                                & \multirow{2}{*}{$k^2 (n^2+1) u$}       & $iku$                                   & $0$                      & $iku$                     \\ \cline{1-4} \cline{6-8}
HH + second order ABC (Sec.~\ref{problem:HH_with_second_order_abcs})  & $H^{1,1}(\Omega, \Gamma)$                       & $-\nabla \cdot (A \nabla u) - k^2 n^2 u$                                 & $-\nabla \cdot (A \nabla u) + k^2 u$                                 &                                         & $\alpha \Delta_\Gamma u + k R_\Gamma u$ & $\alpha \Delta_\Gamma u$ & $k R_\Gamma$              \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Helmholtz (HH) problems covered by the present analysis. The operator $A_\Gamma$ maps into a class of analytic functions, $R_\Gamma$ is an operator of order $0$ bounded uniformly in $k$, $A_\Gamma$ represents an operator mapping into a class of analytic functions. \JMM{[double check the properties of $R_\Gamma$!]} 
}

% % !TEX root = main.tex
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% Model                   &  Energy Space                                   & $\Lkm$                                                                   & $\Lkp$                                                               & $ \TkOmegaM - \TkOmegaP $               & $\TkGammaM$                             & $\TkGammaP$              & $ \TkGammaM - \TkGammaP $ \\ \hline
% HH + RBC                & \multirow{5}{*}{$H^1(\Omega)$}                  & \multirow{3}{*}{$-\nabla \cdot (A \nabla u) - k^2 n^2 u$}                & \multirow{4}{*}{$-\nabla \cdot (A \nabla u) + k^2 u$}                & \multirow{3}{*}{$-k^2(n^2+1)u$}         & $iku$                                   & $0$                      & $iku$                     \\ \cline{1-1} \cline{6-8}
% HH + DtN Sphere         &                                                 &                                                                          &                                                                      &                                         & $\mathrm{DtN}_k$                        & $\mathrm{DtN}_0$         & $k R_\Gamma$              \\ \cline{1-1} \cline{6-8}
% HH + DtN $\Gamma$       &                                                 &                                                                          &                                                                      &                                         & $\mathrm{DtN}_k$                        & $\mathrm{DtN}_0$         & $k R_\Gamma + A_\Gamma$   \\ \cline{1-1} \cline{3-3} \cline{5-8}
% HH + Damping + RBC      &                                                 & $-\nabla \cdot (A \nabla u) - k^2 n^2 u + ikmu$                          &                                                                      & $-k^2(n^2+1)u + ikmu$                   & $iku$                                   & $0$                      & $iku$                     \\ \cline{1-1} \cline{3-8}
% HH + PML + RBC          &                                                 & $-\nabla(A^{PML}_k \nabla u) - k^2 n^2 u$                                & $-\nabla(A^{PML}_k \nabla u) + k^2 u$                                & \multirow{2}{*}{$-k^2 (n^2+1) u$}       & $iku$                                   & $0$                      & $iku$                     \\ \cline{1-4} \cline{6-8}
% HH + second order ABC   & $H^{1,1}(\Omega, \Gamma)$                       & $-\nabla \cdot (A \nabla u) - k^2 n^2 u$                                 & $-\nabla \cdot (A \nabla u) + k^2 u$                                 &                                         & $\alpha \Delta_\Gamma u + k R_\Gamma u$ & $\alpha \Delta_\Gamma u$ & $k R_\Gamma$              \\ \hline
% Elasticity + RBC        & \multirow{2}{*}{$\left[ H^1(\Omega) \right]^d$} & \multirow{2}{*}{$-\nabla \cdot (A \sigma (\pmb{u}) ) - k^2 n^2 \pmb{u}$} & \multirow{2}{*}{$-\nabla \cdot (A \sigma (\pmb{u}) ) + k^2 \pmb{u}$} & \multirow{2}{*}{$-k^2 (n^2+1) \pmb{u}$} & $iku$                                   & $0$                      & $iku$                     \\ \cline{1-1} \cline{6-8}
% Elasticity + DtN Sphere &                                                 &                                                                          &                                                                      &                                         & $\mathrm{DtN}_k$                        & $\mathrm{DtN}_0$         & $k R_\Gamma$              \\ \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Overview table of covered problems.
% }


==> 01_numerical_examples.tex <==
% !TEX root = main.tex
\section{Numerical examples}\label{section:numerical_examples}

All our calculations are performed with the $hp$-FEM code NETGEN/NGSOLVE by J.~Sch\"oberl,~\cite{schoeberlNGSOLVE,schoeberl97}.
The curved boundary and interface are implemented using second order rational splines.
For further detail see the \href{https://ngsolve.org/docu/latest/netgen_tutorials/define_2d_geometries.html?highlight=curved#curved-boundaries}{documentation}.
We plot different errors against $N_\lambda$, the number of degrees of freedom per wavelength,
\begin{equation*}
  N_\lambda = \frac{2 \pi \sqrt[d]{\mathrm{DOF}}}{k \sqrt[d]{\mathrm{|\Omega|}}},
\end{equation*}
where the wavelength $\lambda$ and the wavenumber $k$ are related via $k = 2 \pi / \lambda$ and $\mathrm{DOF}$ denotes the size of the linear system to be solved.

\begin{example}\label{example:smooth_solution}
  Let $\Omega$ be the unit circle in $\mathbb{R}^2$ and consider the problem
  \begin{equation*}
  	\begin{alignedat}{2}
  		- \Delta u - k^2 n^2 u &= 1 \qquad   &&\text{in } \Omega,\\
  		  \partial_n u - i k u &= 0        &&\text{on } \partial \Omega.
  	\end{alignedat}
  \end{equation*}
  The index of refraction $n$ is given in polar coordinates by $n \equiv n_1 \equiv 1$ for $r \leq 1/2$ and $n \equiv n_2 \equiv  2$ for $1/2 < r \leq 1$.
  The exact solution can be derived by elementary calculations.
  In fact, the solution can be derived by separation of variables, in polar coordinates, and is given by
  \[ u(r) = \begin{cases}
        c_1 J_0(k n_1 r) - \frac{1}{(k n_1)^2} & r\leq 1/2, \\
        c_2 J_0(k n_2 r) + c_3 Y_0(k n_2 r) - \frac{1}{(k n_2)^2} & r > 1/2,
     \end{cases}
  \]
  where $J_0$ and $Y_0$ are the Bessel functions of order zero and the constants $c_1$, $c_2$ and $c_3$ can be determined using the Robin boundary conditions as well as the interface conditions.  
  For the numerical studies, we solve this problem using $h$-FEM with polynomial degrees $p = 1$, $2$, $3$ and $4$.
	The results are visualized in Figure \ref{figure:l2_error_rel_hp_fem} for the relative $L^2(\Omega)$ error,
  in Figure \ref{figure:h1_semi_error_rel_hp_fem} for the relative $H^1(\Omega)$ semi-error and
  in Figure \ref{figure:energy_error_rel_hp_fem} for the relative energy error.
	Note that as in the homogeneous case higher order versions are less prone to the pollution effect, see also \cite[Section 4.3]{esterhazy-melenk12}.
\end{example}

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.85\textwidth]{l2_error_rel_hp_fem}
	\caption{
		Numerical results of the $h$-FEM for $p = 1$, $2$, $3$, $4$ as described in Example \ref{example:smooth_solution}.
		The reference line in black corresponds to $h^{p+1}$.
	}
	\label{figure:l2_error_rel_hp_fem}
\end{figure}

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.85\textwidth]{h1_semi_error_rel_hp_fem}
	\caption{
		Numerical results of the $h$-FEM for $p = 1$, $2$, $3$, $4$ as described in Example \ref{example:smooth_solution}.
		The reference line in black corresponds to $h^{p}$.
	}
	\label{figure:h1_semi_error_rel_hp_fem}
\end{figure}


\begin{figure}[ht]
	\centering
	\includegraphics[width=0.85\textwidth]{energy_error_rel_hp_fem}
	\caption{
		Numerical results of the $h$-FEM for $p = 1$, $2$, $3$, $4$ as described in Example \ref{example:smooth_solution}.
		The reference line in black corresponds to $h^{p}$.
	}
	\label{figure:energy_error_rel_hp_fem}
\end{figure}


\noindent
\textbf{Acknowledgement}:
MB is grateful for the financial support by the Austrian Science Fund (FWF) through the doctoral school \textit{Dissipation and dispersion in nonlinear PDEs} (grant W1245).
MB thanks the workgroup of Joachim Sch\"oberl (TU Wien) for help regarding the numerical experiments.


==> 04_adjoint_problems.tex <==
% !TEX root = main.tex
\section{Adjoint problem}\label{section:adjoint_problem}

The proof of quasi-optimality of an abstract Galerkin discretization of
problem \eqref{eq:S_k_minus_problem} hinges on the approximability of the
adjoint problem, i.e., one performs a duality argument.
Below, Lemma~\ref{lemma:characterization_adjoint_problem} will characterize
the solution of the adjoint problem.
The primal problem reads:
\begin{equation*}
  \text{Find } \quad u \eqqcolon \Skm(f,g) \in \HOneT \quad \text{ such that } \quad \bkm(u,v) = (f,v) + \langle g, v\rangle \quad \forall v \in \HOneT.
\end{equation*}
The corresponding adjoint problem reads:
\begin{equation*}
  \text{Find } \quad u^\star \eqqcolon \Skmstar(f,g) \in \HOneT \quad \text{ such that } \quad \bkm(v,u^\star) = (v,f) + \langle v, g\rangle \quad \forall v \in \HOneT.
\end{equation*}
\begin{assumption}[Quasi-selfadjointness of $\TkOmegaM$ and $\TkGammaM$]
  \label{assumption:MINUS_T_k_Omega_Gamma_minus_quasi_selfadjoint}
  The linear operators
  $\TkOmegaM \colon \HOneT \colon \to \HOneT^\prime$
  and
  $\TkGammaM \colon H^{t}(\Gamma) \colon \to H^{-t}( \Gamma)$
  are quasi-selfadjoint, i.e.,
  \begin{align*}
    (\TkOmegaM u, \overline{v}) = (\TkOmegaM v, \overline{u})
    \quad \text{as well as} \quad
    \langle \TkGammaM u, \overline{v} \rangle = \langle \TkGammaM v, \overline{u} \rangle,
  \end{align*}
  for all $u, v \in \HOneT$.
\end{assumption}
For the adjoint problem to be again of the same \textit{character}
one may assume Assumption \ref{assumption:MINUS_T_k_Omega_Gamma_minus_quasi_selfadjoint}.
\begin{lemma}[Adjoint Problems]\label{lemma:characterization_adjoint_problem}
  Let Assumption \ref{assumption:MINUS_T_k_Omega_Gamma_minus_quasi_selfadjoint} be satsified.
  Let $\Skm(f,g; A)$ denote the solution operator specifying the diffusion matrix $A$.
  Then $\Skmstar(f,g) = \overline{\Skm(\overline{f}, \overline{g}; A^T)}$.
\end{lemma}
\begin{proof}
  Let $u^\star = \Skmstar(f,g)$.
  Therefore we have
  \begin{equation}
    (A \nabla v, \nabla u^\star) - (\TkOmegaM v, u^*) - \langle \TkGammaM v, u^\star \rangle
    =
    (v,f) + \langle v, g\rangle \quad \forall v \in \HOneT.
  \end{equation}
  Due to the assume quasi-selfadjointness in Assumption \ref{assumption:MINUS_T_k_Omega_Gamma_minus_quasi_selfadjoint} we find
  \begin{equation}
    (A^T \overline{\nabla u^\star},  \overline{\nabla v}) - (\TkOmegaM \overline{u^\star}, \overline{v}) - \langle \TkGammaM \overline{u^\star},  \overline{v} \rangle
    =
    (\overline{f} , \overline{v}) + \langle \overline{f} , \overline{v} \rangle \quad \forall v \in \HOneT.
  \end{equation}
  Replacing $\overline{v}$ by $v$ we find $\overline{u^\star} = \Skm(\overline{f}, \overline{g}; A^T)$, which yields the result.
\end{proof}
\begin{remark}
  Loosely speaking Lemma \ref{lemma:characterization_adjoint_problem}
  states that under the assumption of quasi-selfadjointness, see Assumption \ref{assumption:MINUS_T_k_Omega_Gamma_minus_quasi_selfadjoint},
  the adjoint problem is again of similar character to the primal problem.
  This in turn is convenient, since the same regularity splitting of Section \ref{section:abstract_contraction_argument}
  can be performed for both the primal and the adjoint problem.
  See also \cite[Lem.~{3.1}]{melenk-sauter11} for similar results in the homogeneous case.
\eremk
\end{remark}
\begin{remark}
  To establish quasi-optimality in Section \ref{section:galerkin} the regularity
  theory developed in Section \ref{section:abstract_contraction_argument} only needs
  to be applicable to the adjoint problem.
  Therefore it is reasonable to introduce the corresponding adjoint operators as well.
  This has the advantage of establishing quasi-optimality as a separate result
  independent of the primal formulation,
  as long as the adjoint problem allows for the application of the results in Section
  \ref{section:abstract_contraction_argument}.
  To that end we introduce the following Definition.
\eremk
\end{remark}
\begin{definition}[Adjoint sesquilinear form $\bkmstar$ and adjoint operators $\TkOmegaMstar$ and $\TkGammaMstar$]
  Given the setting of Section \ref{section:assumptions_and_problem_specific_notation}
  we define the adjoint sesquilinear form $\bkmstar \colon \HOneT \times \HOneT$ by
  \begin{equation*}
    \bkmstar(u,v) = \bkm(v,u), \qquad \forall u,v \in \HOneT.
  \end{equation*}
  The corresponding adjoint operators $\TkOmegaMstar$ and $\TkGammaMstar$ are given by
  \begin{equation*}
    (\TkOmegaMstar u , v) = (\TkOmegaM \overline{v} , \overline{u})
    \quad \text{and} \quad
    \langle \TkGammaMstar u , v \rangle = \langle \TkGammaM \overline{v} , \overline{u} \rangle,
  \end{equation*}
  respectively.
\end{definition}


==> 07_numerical_examples.tex <==
% !TEX root = main.tex
\section{Numerical examples}\label{section:numerical_examples}
%--------------------------------------
\JMM{[todo: didn't we want to include some numerics on the sharpness of the log k?]}

All our calculations are performed with the $hp$-FEM code NETGEN/NGSOLVE by J.~Sch\"oberl,~\cite{schoeberlNGSOLVE,schoeberl97}.
The curved boundary and interface are implemented using second order rational splines.
We plot different errors against $N_\lambda$, the number of degrees of freedom per wavelength,
\begin{equation*}
  N_\lambda = \frac{2 \pi \sqrt[d]{\mathrm{DOF}}}{k \sqrt[d]{\mathrm{|\Omega|}}},
\end{equation*}
where the wavelength $\lambda$ and the wavenumber $k$ are related via $k = 2 \pi / \lambda$ and $\mathrm{DOF}$ denotes the size of the linear system to be solved.

\begin{example}\label{example:smooth_solution}
  Let $\Omega$ be the unit circle in $\mathbb{R}^2$ and consider the problem
  \begin{equation*}
  	\begin{alignedat}{2}
  		- \Delta u - k^2 n^2 u &= 1 \qquad   &&\text{in } \Omega,\\
  		  \partial_n u - i k u &= 0        &&\text{on } \partial \Omega.
  	\end{alignedat}
  \end{equation*}
  The index of refraction $n$ is given in polar coordinates by $n \equiv n_1 \equiv 1$ for $r \leq 1/2$ and $n \equiv n_2 \equiv  2$ for $1/2 < r \leq 1$.
  The exact solution can be derived by elementary calculations.
  In fact, the solution can be derived by separation of variables, in polar coordinates, and is given by
  \[ u(r) = \begin{cases}
        c_1 J_0(k n_1 r) - \frac{1}{(k n_1)^2} & r\leq 1/2, \\
        c_2 J_0(k n_2 r) + c_3 Y_0(k n_2 r) - \frac{1}{(k n_2)^2} & r > 1/2,
     \end{cases}
  \]
  where $J_0$ and $Y_0$ are the Bessel functions of order zero and the constants $c_1$, $c_2$ and $c_3$ can be determined using the Robin boundary conditions as well as the interface conditions.
  For the numerical studies, we solve this problem using $h$-FEM with polynomial degrees $p = 1$, $2$, $3$ and $4$.
  It is important to note that the interface $\interface$ is resolved by the mesh.
  Therefore, the observed rates are optimal with respect to the employed finite element space, since the solution is piecewise smooth.
	The results are visualised in Figure \ref{figure:l2_error_and_energy_error_rel_hp_fem}.
	Note that as in the homogeneous case higher order versions are less prone to the pollution effect, see also \cite[Section 4.3]{esterhazy-melenk12}.
\end{example}

\begin{figure}[!ht]%
    \centering
		{	\includegraphics[width=0.48\textwidth]{fig/l2_error_rel_hp_fem} }%
    \quad
		{ \includegraphics[width=0.48\textwidth]{fig/energy_error_rel_hp_fem} }%
		\caption{
    Numerical results of the $h$-FEM for $p = 1$, $2$, $3$, $4$ as described in Example \ref{example:smooth_solution}.
    Relative $L^2(\Omega)$ error (left) with reference line in black corresponding to $h^{p+1}$.
    Relative energy error (right) with reference line in black corresponding to $h^{p}$.
		}%
		\label{figure:l2_error_and_energy_error_rel_hp_fem}%
\end{figure}

% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{fig/l2_error_rel_hp_fem}
% 	\caption{
% 		Numerical results of the $h$-FEM for $p = 1$, $2$, $3$, $4$ as described in Example \ref{example:smooth_solution}.
% 		The reference line in black corresponds to $h^{p+1}$.
% 	}
% 	\label{figure:l2_error_rel_hp_fem}
% \end{figure}
%
% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{fig/h1_semi_error_rel_hp_fem}
% 	\caption{
% 		Numerical results of the $h$-FEM for $p = 1$, $2$, $3$, $4$ as described in Example \ref{example:smooth_solution}.
% 		The reference line in black corresponds to $h^{p}$.
% 	}
% 	\label{figure:h1_semi_error_rel_hp_fem}
% \end{figure}
%
% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.85\textwidth]{fig/energy_error_rel_hp_fem}
% 	\caption{
% 		Numerical results of the $h$-FEM for $p = 1$, $2$, $3$, $4$ as described in Example \ref{example:smooth_solution}.
% 		The reference line in black corresponds to $h^{p}$.
% 	}
% 	\label{figure:energy_error_rel_hp_fem}
% \end{figure}
%
% \begin{example}\label{example:smooth_solution_corner_interface}
%   Let $\Omega$ be the unit circle in $\mathbb{R}^2$ and
%   $\Gamma_i$ the quadrilateral with corners $(-1/2, -1/2)$, $(1/2, -1/2)$, $(-1/2, 1/2)$ and $(1/2, 1/2)$.
%   The index of refraction $n$ is given by $n \equiv n_1 \equiv 1$ inside of $\Gamma_i$ and $n \equiv n_2 \equiv  2$ otherwise.
%   We choose as the exact solution
%   \begin{equation*}
%   	\begin{alignedat}{2}
%   		- \Delta u - k^2 n^2 u &= f \qquad   &&\text{in } \Omega,\\
%   		\partial_n u - i k u &= g        &&\text{on } \partial \Omega.
%   	\end{alignedat}
%   \end{equation*}
%   where the data $f$ and $g$ are such that the exact solution is given by $u(x,y) = \mathrm{e}^{i(k_1 x + k_2 y)}$ with $k_1 = - k_2 = \frac{1}{\sqrt{2}} k$.
% 	For the numerical studies, this problem will be solved using $h$-FEM with polynomial degrees $p = 1$, $2$, $3$ and $4$.
%   Again the interface $\Gamma_i$ is resolved by the mesh.
%   The results are visualised in Figure \ref{figure:l2_error_and_energy_error_rel_hp_fem_corner_interface}.
% \end{example}
%
% \begin{figure}[!ht]%
%     \centering
% 		{	\includegraphics[width=0.48\textwidth]{fig/l2_error_rel_hp_fem_corner_interface} }%
%     \quad
% 		{ \includegraphics[width=0.48\textwidth]{fig/energy_error_rel_hp_fem_corner_interface} }%
% 		\caption{
%     Numerical results of the $h$-FEM for $p = 1$, $2$, $3$, $4$ as described in \ref{example:smooth_solution_corner_interface}.
%     Relative $L^2(\Omega)$ error (left) with reference line in black corresponding to $h^{p+1}$.
%     Relative energy error (right) with reference line in black corresponding to $h^{p}$.
% 		}%
% 		\label{figure:l2_error_and_energy_error_rel_hp_fem_corner_interface}%
% \end{figure}
%
%
% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.85\textwidth]{fig/l2_error_rel_hp_fem_corner_interface}
% 	\caption{
% 		Numerical results of the $h$-FEM for $p = 1$, $2$, $3$, $4$ as described in Example \ref{example:smooth_solution_corner_interface}.
% 		The reference line in black corresponds to $h^{p+1}$.
% 	}
% 	\label{figure:l2_error_rel_hp_fem_corner_interface}
% \end{figure}
%
% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.85\textwidth]{fig/h1_semi_error_rel_hp_fem_corner_interface}
% 	\caption{
% 		Numerical results of the $h$-FEM for $p = 1$, $2$, $3$, $4$ as described in Example \ref{example:smooth_solution_corner_interface}.
% 		The reference line in black corresponds to $h^{p}$.
% 	}
% 	\label{figure:h1_semi_error_rel_hp_fem_corner_interface}
% \end{figure}
%
% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.85\textwidth]{fig/energy_error_rel_hp_fem_corner_interface}
% 	\caption{
% 		Numerical results of the $h$-FEM for $p = 1$, $2$, $3$, $4$ as described in Example \ref{example:smooth_solution_corner_interface}.
% 		The reference line in black corresponds to $h^{p}$.
% 	}
% 	\label{figure:energy_error_rel_hp_fem_corner_interface}
% \end{figure}


\begin{example}\label{example:smooth_second_order_abcs_solution}
  Let again $\Omega$ be the unit circle in $\mathbb{R}^2$ and consider the problem
  \begin{equation*}
  	\begin{alignedat}{2}
  		- \Delta u - k^2 n^2 u &= f \qquad   &&\text{in } \Omega,\\
  		  \partial_n u - \alpha \Delta_\Gamma u - \beta u &= g        &&\text{on } \partial \Omega.
  	\end{alignedat}
  \end{equation*}
  The index of refraction $n$ is given in polar coordinates by $n \equiv n_1 \equiv 1$ for $r \leq 1/2$ and $n \equiv n_2 \equiv  2$ for $1/2 < r \leq 1$.
  The parameters $\alpha$ and $\beta$ are chosen according to \cite{feng83}:
  \begin{equation*}
    \alpha = -\frac{i}{2k}
    \qquad
    \beta  = i k - \frac{1}{2} - \frac{i}{8k}
  \end{equation*}
  The exact solution is chosen to be $u(x,y) = \sin(k(x+y))$.
  The right hand sides $f$ and $g$ are calculated accordingly.
  Note that on the unit sphere the surface gradient can be expressed
  for sufficiently smooth functions as the trace of $(-y, x)^T \cdot \nabla u$,
  which allows for staightforward numerical discretization of the problem in question.
  For the numerical studies, we solve this problem using $h$-FEM with polynomial degrees $p = 1$, $2$, $3$ and $4$.
  It is important to note that the interface $\interface$ is resolved by the mesh.
  Therefore, the observed rates are optimal with respect to the employed finite element space, since the solution is piecewise smooth.
	The results are visualised in Figure \ref{figure:l2_error_and_energy_error_rel_s_second_order_abc_hp_fem}.
\end{example}

\begin{figure}[!ht]%
    \centering
		{	\includegraphics[width=0.48\textwidth]{fig/l2_error_rel_second_order_abc_hp_fem} }%
    \quad
		{ \includegraphics[width=0.48\textwidth]{fig/energy_error_rel_with_surf_second_order_abc_hp_fem} }%
		\caption{
    Numerical results of the $h$-FEM for $p = 1$, $2$, $3$, $4$ as described in Example \ref{example:smooth_second_order_abcs_solution}.
    Relative $L^2(\Omega)$ error (left) with reference line in black corresponding to $h^{p+1}$.
    Relative energy error (right) with reference line in black corresponding to $h^{p}$.
		}%
		\label{figure:l2_error_and_energy_error_rel_s_second_order_abc_hp_fem}%
\end{figure}


==> 09_dtn_elasticity.tex <==
% !TEX root = main.tex
\section{DtN for Elsticity}

Following the notation and assumptions of \cite{brown_gallistl16},
we denote by $\lambda$ and $\mu$ the Lame parameters.
We assume $\mu > 0$ and $\lambda \geq 0$, which is common for elastic materials,
see \cite[p. 299]{mclean00}.
We stress however that our results hold for a larger set of parameters,
it would suffice to assume $\mu > 0$ and $\lambda + \frac{5}{3}\mu \geq 0$.
We denote by $J_{\nu}$ and $Y_{\nu}$ the standard Bessel functions.
Furthermore, the Hankel function $H^{(1)}_{\nu}$ is given by
$H^{(1)}_{\nu} = J_{\nu} + i Y_{\nu}$.
The Dirichlet-to-Neumann map is explicitly known on the sphere.
We follow \cite{yuan19}.
See \cite[Equation 2.59]{yuan19}, where an explicit formula in spatial dimension two is given.
With $R=1$, i.e., on the unit sphere, and in our notation with $k$ instead of $\omega$ we have
\begin{align*}
  \mathrm{DtN}_k \pmb{u}
  &=
  \sum_{n \in \mathbb{Z}}
  \left[
    \left( -\mu + \frac{\alpha_{2,n} k^2}{\Lambda_n} \right) u_n^r
    +
    \left( -in\mu + \frac{i n k^2}{\Lambda_n} \right) u_n^\theta
  \right] \pmb{e}_r \mathrm{e}^{in\theta} \\
  &+
  \sum_{n \in \mathbb{Z}}
  \left[
    \left( -\mu + \frac{\alpha_{1,n} k^2}{\Lambda_n} \right) u_n^\theta
    +
    \left( in\mu - \frac{i n k^2}{\Lambda_n} \right) u_n^r
  \right] \pmb{e}_\theta \mathrm{e}^{in\theta}
\end{align*}
where $\Lambda_n$ is given by, see again \cite[Last equation of Proof of Lemma 2.7.1]{yuan19}
\begin{equation*}
  \Lambda_n = n^2 - \alpha_{1,n} \alpha_{2,n}
\end{equation*}
with, see \cite[second to last equation of Proof of Lemma 2.7.1]{yuan19}
\begin{equation*}
  \alpha_{1,n} =
  \kappa_1 \frac{ H_n^{(1) \prime} (\kappa_1) }{H_n^{(1)} (\kappa_1)}
  \qquad
  \alpha_{2,n} =
  \kappa_2 \frac{ H_n^{(1) \prime} (\kappa_2) }{H_n^{(1)} (\kappa_2)}
\end{equation*}
with compressional and shear wavenumber $\kappa_1$ and $\kappa_2$ given
\begin{equation*}
  \kappa_1  = \frac{k}{\sqrt{\lambda + 2 \mu}}
  \qquad
  \kappa_2  = \frac{k}{\sqrt{\mu}}
\end{equation*}
with $\lambda, \mu$ being the Lame Parameter, see
\cite[Page 10, between equation 2.3 and 2.4]{yuan19}.
The canonical operator $\mathrm{DtN}_0$ is derived by considering the
symbol of $\mathrm{DtN}_k$ and passing to $k=0$.
We now state some properties of Hankel functions:
\begin{lemma}[Properties of Hankel functions]
  There holds:
  \begin{enumerate}
    \item $H_{-n}^{(1)} = (-1)^n H_{n}^{(1)}$.
    \item $H_{0}^{(1)}(z) \sim \frac{2 i}{\pi} \ln z$ for $z \to 0$.
    \item $H_{n}^{(1)}(z) \sim - \frac{i}{\pi} \Gamma(n) \left( \frac{z}{2} \right)^{-n}$ for $n > 0$ and $z \to 0$.
  \end{enumerate}
\end{lemma}
\begin{lemma}[Properties of Symbol]
  There holds:
  \begin{itemize}
    \item $\alpha_{i,-n} = \alpha_{i,n}$ for $i = 1$, $2$.
    \item $\alpha_{i,n} \rightarrow -|n|$ for $k \to 0$.
    \item $\frac{k^2}{\Lambda_0} \rightarrow 0$ for $k \to 0$.
    \item $\frac{k^2}{\Lambda_n} \rightarrow \frac{2 \mu (\lambda + 2 \mu) (|n| - 1)}{(\lambda + 3 \mu) |n|}$ for $k \to 0$ and $n \geq 1$.
  \end{itemize}
\end{lemma}
We therefore find
\begin{align*}
  \left( -\mu + \frac{\alpha_{2,n} k^2}{\Lambda_n} \right) &\rightarrow  -\mu - \sigma_n, \\
  \left( -in\mu + \frac{i n k^2}{\Lambda_n} \right)        &\rightarrow  - i n \mu  + i \mathrm{sgn}(n) \sigma_n,      \\
  \left( -\mu + \frac{\alpha_{1,n} k^2}{\Lambda_n} \right) &\rightarrow  -\mu - \sigma_n, \\
  \left( in\mu - \frac{i n k^2}{\Lambda_n} \right)         &\rightarrow   i n \mu  - i \mathrm{sgn}(n) \sigma_n,
\end{align*}
with
\[
\sigma_n \coloneqq
\begin{cases}
  0 & n=0 \\
  \frac{2 \mu (\lambda + 2 \mu)}{ (\lambda + 3 \mu) } (|n| - 1) & \text{else}
\end{cases}
\]
where we used $\alpha_{1,n} \rightarrow -|n|$ and $\alpha_{2,n} \rightarrow -|n|$
We therefore find the correct choice of $\mathrm{DtN}_0$ to be
\begin{align*}
  \mathrm{DtN}_0 \pmb{u}
  &=
  \sum_{n \in \mathbb{Z}}
  \left[
    \left( -\mu - \sigma_n \right) u_n^r
    +
    \left( - i n \mu  + i \mathrm{sgn}(n) \sigma_n \right) u_n^\theta
  \right] \pmb{e}_r \mathrm{e}^{in\theta} \\
  &+
  \sum_{n \in \mathbb{Z}}
  \left[
    \left( -\mu - \sigma_n \right) u_n^\theta
    +
    \left( i n \mu  - i \mathrm{sgn}(n) \sigma_n  \right) u_n^r
  \right] \pmb{e}_\theta \mathrm{e}^{in\theta}.
\end{align*}
\begin{lemma}[Positivity of $-\mathrm{DtN}_0$]
  Let $\lambda + \frac{5}{3}\mu \geq 0$.
  Then the operator $-\mathrm{DtN}_0$ is positive, i.e.,
  \begin{equation*}
    - \langle \mathrm{DtN}_0 u , u \rangle \geq 0,
  \end{equation*}
  for all $u \in H^{1/2}(\Gamma)$.
\end{lemma}
\begin{proof}
  The positivity of $-\mathrm{DtN}_0$ follows immediately
  from the positive definiteness of the matrix corresponding to the symbol.
  Hence, once we find the for each $n \in \mathbb{Z}$ matrix
  \begin{equation*}
    M_n \coloneqq -
    \begin{pmatrix}
       -\mu - \sigma_n & - i n \mu  + i \mathrm{sgn}(n) \sigma_n \\
      i n \mu  - i \mathrm{sgn}(n) \sigma_n &  -\mu - \sigma_n  \\
    \end{pmatrix}
  \end{equation*}
  to be positive definite, the proof is complete.
  For $n = 0$ we have
  \begin{equation*}
    M_0 =
    \begin{pmatrix}
      \mu  & 0 \\
      0 & \mu \\
    \end{pmatrix}
  \end{equation*}
  which is trivially positive definite, since $\mu > 0$.
  For $n \neq 0$ we have
  \begin{equation*}
    M_n =
    \begin{pmatrix}
      \mu + \frac{2 \mu (\lambda + 2 \mu)}{ (\lambda + 3 \mu) } (|n| - 1) & - i n \mu  + i \mathrm{sgn}(n) \frac{2 \mu (\lambda + 2 \mu)}{ (\lambda + 3 \mu) } (|n| - 1) \\
      i n \mu  - i \mathrm{sgn}(n) \frac{2 \mu (\lambda + 2 \mu)}{ (\lambda + 3 \mu) } (|n| - 1) & \mu + \frac{2 \mu (\lambda + 2 \mu)}{ (\lambda + 3 \mu) } (|n| - 1) \\
    \end{pmatrix}
  \end{equation*}
  Since $\mu > 0$ and $\lambda + \frac{5}{3} \mu$ we find
  \begin{equation*}
    \mu + \frac{2 \mu (\lambda + 2 \mu)}{ (\lambda + 3 \mu) } (|n| - 1) \geq 0,
  \end{equation*}
  hence, the top-left entry of $M_n$ is positive for $n \in \mathbb{Z} \setminus \{0\}$.
  It is easily verified that in fact the determinant is also positive under the assumptions of the present lemma,
  which concludes the proof.
\end{proof}
The difference $\mathrm{DtN}_k - \mathrm{DtN}_0$ is given by
\begin{align*}
  \mathrm{DtN}_k \pmb{u} - \mathrm{DtN}_0 \pmb{u}
  &=
  \sum_{n \in \mathbb{Z}}
  \left[
    \left( \frac{\alpha_{2,n} k^2}{\Lambda_n} + \sigma_n \right) u_n^r
    +
    \left( \frac{i n k^2}{\Lambda_n} - i \mathrm{sgn}(n) \sigma_n \right) u_n^\theta
  \right] \pmb{e}_r \mathrm{e}^{in\theta} \\
  &+
  \sum_{n \in \mathbb{Z}}
  \left[
    \left( \frac{\alpha_{1,n} k^2}{\Lambda_n} + \sigma_n \right) u_n^\theta
    +
    \left( - \frac{i n k^2}{\Lambda_n} + i \mathrm{sgn}(n) \sigma_n  \right) u_n^r
  \right] \pmb{e}_\theta \mathrm{e}^{in\theta}.
\end{align*}
We are going to split the difference again additively into an operator
of order zero and an operator which maps into analytic functions.
This is done by splitting the series representation into a high and low frequency component:
\begin{equation*}
  \mathrm{DtN}_k \pmb{u} - \mathrm{DtN}_0 \pmb{u}
  = \sum_{n \in \mathbb{Z}} \cdots
  = \sum_{|n| > 2k} \cdots + \sum_{|n| \leq 2k} \cdots
  = R_\Gamma + A_\Gamma
\end{equation*}
We first analyze the operator $R_\Gamma$.
To that end, as in the proof of Lemma \ref{lemma:properties_dtn_operators_sphere} it suffices to estimate the symbol.
Hence, once we have shown
\begin{align*}
  \left| \frac{\alpha_{2,n} k^2}{\Lambda_n} + \sigma_n \right| &\lesssim k \\
  \left| \frac{\alpha_{1,n} k^2}{\Lambda_n} + \sigma_n \right| &\lesssim k \\
  \left| \frac{i n k^2}{\Lambda_n} - i \mathrm{sgn}(n) \sigma_n \right| &\lesssim k \\
\end{align*}
for $n \geq 2k$, uniformly in $n$, we can conclude $R_\Gamma$ have the mapping properties as in Lemma \ref{lemma:properties_dtn_operators_sphere}.
To that end we analyze the asymptotic behavior of
\begin{equation*}
  x \frac{ H_n^{(1) \prime} (x) }{H_n^{(1)} (x)}
\end{equation*}
for $n \geq 2x$ and large $n$.
Since $H_n^{(1)} = J_n + i Y_n$ and $Y_n$ is the dominant part we find that for $n \geq 2x$
\begin{equation*}
  x \frac{ H_n^{(1) \prime} (x) }{H_n^{(1)} (x)} \sim  x \frac{ Y_n^{\prime} (x) }{Y_n (x)}.
\end{equation*}
We now apply the uniform asymptotic expansions for $Y_n$ and $Y_n^{\prime}$ given in the \cite[Eq.~10.20.5]{DLMF} for $Y_n$ and \cite[Eq.~10.20.8]{DLMF} for $Y_n^{\prime}$ with $z=x/n$ and
\begin{equation}\label{eq:connecting_formulas_bessel_asymptotics}
  z=\frac{x}{n} \quad \text{ and } \quad \frac{2}{3}\zeta^{3/2} = \ln \frac{1+\sqrt{1-z^2}}{z} - \sqrt{1-z^2}
\end{equation}
we have
\begin{align*}
  Y_n (z) &\sim -\left(\frac{4\zeta}{1-z^{2}}\right)^{\frac{1}{4}}\left(\frac{\mathrm{Bi}\left(\nu^{\frac{2}{3}}\zeta\right)}{\nu^{\frac{1}{3}}}\sum_{k=0}^{\infty}\frac{A_{k}(\zeta)}{\nu^{2k}}+\frac{\mathrm{Bi}'\left(\nu^{\frac{2}{3}}\zeta\right)}{\nu^{\frac{5}{3}}}\sum_{k=0}^{\infty}\frac{B_{k}(\zeta)}{\nu^{2k}}\right) \\
  Y_n^{\prime} (z) &\sim \frac{2}{z}\left(\frac{1-z^{2}}{4\zeta}\right)^{\frac{1}{4}}\*\left(\frac{\mathrm{Bi}\left(\nu^{\frac{2}{3}}\zeta\right)}{\nu^{\frac{4}{3}}}\sum_{k=0}^{\infty}\frac{C_{k}(\zeta)}{\nu^{2k}}+\frac{\mathrm{Bi}'\left(\nu^{\frac{2}{3}}\zeta\right)}{\nu^{\frac{2}{3}}}\sum_{k=0}^{\infty}\frac{D_{k}(\zeta)}{\nu^{2k}}\right)
\end{align*}
Expaning the Airy functions as well as truncating the above series expansions we find after simplifying
\begin{equation*}
  x \frac{ Y_n^{\prime} (x) }{Y_n (x)} \sim - \sqrt{n^2 - x^2} \frac{n-V_1(p)}{n-U_1(p)},
\end{equation*}
with
\begin{align*}
  p   &= (1 - z^2)^{-1/2} \\
  U_1 &= \frac{1}{24} (3p-5p^3) \\
  V_1 &= \frac{1}{24} (-9p+7p^3)
\end{align*}
Taylor expanding we find
\begin{equation*}
  \frac{n-V_1(p)}{n-U_1(p)} = 1+O\left(\frac{x^2}{n^3}\right).
\end{equation*}
Finally,
\begin{align*}
  x \frac{ Y_n^{\prime} (x) }{Y_n (x)}
  &= - \sqrt{n^2 - x^2} \left( 1+O(\frac{x^2}{n^3}) \right) \\
  &= - n \left(1 - \frac{x^2}{2n^2} + O\left(\frac{x^4}{n^4}\right) \right) \left( 1+O\left(\frac{x^2}{n^3}\right) \right) \\
  &= - n \left(1 - \frac{x^2}{2n^2} + O\left(\frac{x^4}{n^4}\right) \right) \left( 1+O\left(\frac{x^2}{n^3}\right) \right) \\
  &= - n + \frac{x^2}{2n^2} + r
\end{align*}
with
\begin{equation*}
  |r| \lesssim \frac{x^2}{n^2} + \frac{x^4}{n^3}.
\end{equation*}
In summary we have
\begin{equation*}
  \alpha_{i,n}
  = - n + \frac{\kappa_i^2}{2n} + r_i.
\end{equation*}
with $|r_i| \lesssim \frac{x^2}{n^2} + \frac{x^4}{n^3}$.
We want the symbol of $\mathrm{DtN}_k - \mathrm{DtN}_0$ for $n \geq 2k$ to be bounded independently of $n$ by one power of $k$.
In particular we want
\begin{equation*}
  \left| \frac{n k^2}{\Lambda_n} - \sigma_n \right| \lesssim k
\end{equation*}
Since $\sigma_n = \frac{2 \mu (\lambda + 2 \mu)}{ (\lambda + 3 \mu) } (|n| - 1)$,
let us introduce $\widehat{\sigma} = \frac{2 \mu (\lambda + 2 \mu)}{ (\lambda + 3 \mu) }$.
Hence
\begin{equation*}
  \left| \frac{n k^2}{\Lambda_n} - \sigma_n \right| \lesssim k
  \qquad \text{is equivalent to} \qquad
  \left| \frac{k^2}{\Lambda_n} - \widehat{\sigma} \right| \lesssim \frac{k}{n}.
\end{equation*}
We now use the asymptotics for $\alpha_{i,n}$ to find
\begin{equation*}
  \alpha_{1,n} \alpha_{2,n}
  = n^2 - \frac{\kappa_1^2 + \kappa_2^2}{2} + \frac{\kappa_1^2 \kappa_2^2}{4n^2} - n(r_1 + r_2) + \frac{\kappa_1^2}{2n} r_2 + \frac{\kappa_2^2}{2n} r_1 + r_1 r_2
\end{equation*}
Note that
\begin{equation*}
  \frac{\kappa_1^2 + \kappa_2^2}{2} = k^2 \frac{1}{\widehat{\sigma}}
\end{equation*}
and therefore
\begin{equation*}
  \alpha_{1,n} \alpha_{2,n}
  = n^2 - k^2 \frac{1}{\widehat{\sigma}} + \frac{\kappa_1^2 \kappa_2^2}{4n^2} - n(r_1 + r_2) + \frac{\kappa_1^2}{2n} r_2 + \frac{\kappa_2^2}{2n} r_1 + r_1 r_2
\end{equation*}
We calculate
\begin{align*}
  \frac{k^2}{\Lambda_n} - \widehat{\sigma}
  &=
  \frac{k^2}{n^2 - \alpha_{1,n} \alpha_{2,n}} - \widehat{\sigma} \\
  &=
  \frac{k^2}{n^2 - n^2 + k^2 \frac{1}{\widehat{\sigma}} - \frac{\kappa_1^2 \kappa_2^2}{4n^2} + n(r_1 + r_2) - \frac{\kappa_1^2}{2n} r_2 - \frac{\kappa_2^2}{2n} r_1 - r_1 r_2 } - \widehat{\sigma}  \\
  &=
  \frac{k^2}{\frac{k^2}{\widehat{\sigma}} - \frac{\kappa_1^2 \kappa_2^2}{4n^2} + n(r_1 + r_2) - \frac{\kappa_1^2}{2n} r_2 - \frac{\kappa_2^2}{2n} r_1 - r_1 r_2 } - \widehat{\sigma}  \\
\end{align*}
Factorizing the denominator we find
\begin{align*}
  \frac{k^2}{\Lambda_n} - \widehat{\sigma}
  &=
  \frac{k^2}{\frac{k^2}{\widehat{\sigma}} (1 + \rho) } - \widehat{\sigma}  \\
  &=
  - \widehat{\sigma}\frac{\rho}{1 + \rho}
\end{align*}
with $\rho$ given by
\begin{equation*}
  \rho
  = \frac{\widehat{\sigma}}{k^2} \left( - \frac{\kappa_1^2 \kappa_2^2}{4n^2} + n(r_1 + r_2) - \frac{\kappa_1^2}{2n} r_2 - \frac{\kappa_2^2}{2n} r_1 - r_1 r_2 \right)
\end{equation*}
Hence we want
\begin{equation*}
  | \rho | \lesssim \frac{k}{n}
\end{equation*}
This leads to the conditions
\begin{align*}
  \left| \frac{\kappa_1^2 \kappa_2^2}{4n^2k^2} \right| &\lesssim  \frac{k}{n} \\
  \left| \frac{n(r_1 + r_2)}{k^2} \right| &\lesssim  \frac{k}{n} \\
  \left|  \frac{\kappa_1^2}{2nk^2} r_2 \right| &\lesssim  \frac{k}{n} \\
  \left|  \frac{\kappa_2^2}{2nk^2} r_1 \right| &\lesssim  \frac{k}{n} \\
  \left| \frac{r_1 r_2}{k^2} \right| &\lesssim  \frac{k}{n} \\
\end{align*}
Note that the first one in the above is satisfied since $n \geq 2k$.
Simplifying the above leads to the conditions
\begin{align*}
  \left| r_i \right| &\lesssim  \frac{k^3}{n^2} \\
  \left| r_i \right| &\lesssim  k \\
  \left| r_1 r_2 \right| &\lesssim  \frac{k^3}{n} \\
\end{align*}
with the first one implying the others.
By the previous analysis we find the first estimate to be true, which concludes the analysis of the symbol.
% \TODO{THIS IS LEGACY STUFF:
% \begin{equation}\label{eq:compound_asymptotic_bessel_j}
%   J_{\nu}(\nu z)
%   \sim
%   \frac{1}{\nu^{1/3}}
%   \left( \frac{4 \zeta}{1-z^2} \right)^{1/4}
%   \left\{
%     \mathrm{Ai}( \nu^{2/3} \zeta ) \sum_{s=0}^\infty \frac{A_s(\zeta)}{\nu^{2s}}
%     +
%     \frac{\mathrm{Ai}^\prime( \nu^{2/3} \zeta )}{\nu^{4/3}} \sum_{s=0}^\infty \frac{B_s(\zeta)}{\nu^{2s}} \right\}
% \end{equation}
% \begin{equation}\label{eq:compound_asymptotic_bessel_y}
%   Y_{\nu}(\nu z)
%   \sim
%   -\frac{1}{\nu^{1/3}}
%   \left( \frac{4 \zeta}{1-z^2} \right)^{1/4}
%   \left\{
%     \mathrm{Bi}( \nu^{2/3} \zeta ) \sum_{s=0}^\infty \frac{A_s(\zeta)}{\nu^{2s}}
%     +
%     \frac{\mathrm{Bi}^\prime( \nu^{2/3} \zeta )}{\nu^{4/3}} \sum_{s=0}^\infty \frac{B_s(\zeta)}{\nu^{2s}} \right\}
% \end{equation}
% \begin{equation}\label{eq:connecting_formulas_bessel_asymptotics}
%   \frac{2}{3}\zeta^{3/2} = \ln \frac{1+\sqrt{1-z^2}}{z} - \sqrt{1-z^2}
% \end{equation}
% uniformly in $z$.
% Furthermore,
% \begin{equation}\label{eq:def_A_in_bessel_asymp}
%   A_{k}(\zeta)
%   =
%   \sum_{j=0}^{2k}
%   \left(\frac{3}{2}\right)^{j}
%   v_{j}
%   \zeta^{-3j/2}
%   U_{2k-j}(p)
% \end{equation}
% \begin{equation}\label{eq:def_A_in_bessel_asymp}
%   B_{k}(\zeta)
%   =
%   -\zeta^{-\frac{1}{2}}
%   \sum_{j=0}^{2k+1}
%   \left(\frac{3}{2}\right)^{j}
%   u_{j}
%   \zeta^{-3j/2}
%   U_{2k-j+1}(p)
% \end{equation}
% with $p=(1+z^{2})^{-\frac{1}{2}}$
% \begin{align*}
%   U_{0}(p)
%   &= 1\\
%   U_{1}(p)
%   &= \frac{1}{24}(3p-5p^{3})\\
%   U_{2}(p)
%   &= \frac{1}{1152}(81p^{2}-462p^{4}+385p^{6})\\
%   U_{3}(p)
%   &= \frac{1}{414720}(30375p^{3}-369603p^{5}+765765p^{7}-425425p^{9})
% \end{align*}
% Hence we find:
% \begin{equation*}
%   \begin{alignedat}{2}
%     A_{0}(\zeta)
%     &= 1  \qquad
%     B_{0}(\zeta)
%     &&= -\zeta^{-\frac{1}{2}}\left(U_{1}(p) + \frac{3}{2} u_{1} \zeta^{-3/2}\right)\\
%     A_{1}(\zeta) &= 1234  \qquad B_{1}(\zeta) &&= 1234
%   \end{alignedat}
% \end{equation*}
% The following asymptotics hold for the Airy functions:
% \begin{equation}\label{eq:zeta_airy}
%   \xi = \frac{2}{3} z^{\frac{3}{2}}
% \end{equation}
% with $u_0 = v_0 = 1$
% \begin{equation}\label{eq:u_k_airy}
%   u_k = \frac{(2k+1)(2k+3)(2k+5)\cdots(6k-1)}{216^{k}k!}=\frac{(6k-5)(6k-3)(6k-1)}{(2k-1)216k}u_{k-1}
% \end{equation}
% \begin{equation}\label{eq:v_k_airy}
%   v_k = \frac{6k+1}{1-6k}u_{k}
% \end{equation}
% \begin{equation}\label{eq:Airy_A}
%   \mathrm{Ai}(z)
%   \sim
%   \frac{e^{-\xi}}{2\sqrt{\pi}z^{1/4}}\sum_{k=0}^{\infty}(-1)^{k}\frac{u_{k}}{\xi^{k}}
% \end{equation}
% \begin{equation}\label{eq:Airy_A_prime}
%   \mathrm{Ai}^\prime(z)
%   \sim
%   -\frac{z^{1/4}e^{-\xi}}{2\sqrt{\pi}}\sum_{k=0}^{\infty}(-1)^{k}\frac{v_{k}}{\xi^{k}}
% \end{equation}
% \begin{equation}\label{eq:Airy_B}
%   \mathrm{Bi}(z)
%   \sim
%   \frac{e^{\xi}}{\sqrt{\pi}z^{1/4}}\sum_{k=0}^{\infty}\frac{u_{k}}{\xi^{k}}
% \end{equation}
% \begin{equation}\label{eq:Airy_B_prime}
%   \mathrm{Bi}^\prime(z)
%   \sim
%   \frac{z^{1/4}e^{\xi}}{\sqrt{\pi}}\sum_{k=0}^{\infty}\frac{v_{k}}{\xi^{k}}
% \end{equation}
% We are interested in
% \begin{equation}
%   M_{\nu}(x)
%   =
%   \frac{J_{\nu}(x)J_{\nu+1}(x) + Y_{\nu}(x)Y_{\nu+1}(x)}{J_{\nu}^2(x) + Y_{\nu}^2(x)}
% \end{equation}
% Hence we consider now
% \begin{equation}
%   \frac{J_{\nu}(\nu z_1)J_{\mu}( \mu z_2 ) + Y_{\nu}(\nu z_1)Y_{\mu}( \mu z_2 )}{J_{\nu}^2(\nu z_1) + Y_{\nu}^2(\nu z_1)}
% \end{equation}
% with the later choice
% \begin{equation}
%   z_1 = \frac{x}{\nu} \quad \mu = \nu + 1 \quad z_2 = \frac{x}{\mu} = \frac{x}{\nu+1}
% \end{equation}
% We first estimate
% \begin{equation}
%   \frac{Y_{\nu}(\nu z_1)Y_{\mu}( \mu z_2 )}{J_{\nu}^2(\nu z_1) + Y_{\nu}^2(\nu z_1)}
% \end{equation}
% To that end let us simplify the asymptotics for $J$ and $Y$:
% \begin{equation}\label{eq:compound_asymptotic_bessel_j_first_order}
%   J_{\nu}(\nu z)
%   \sim
%   \frac{1}{\nu^{1/3}}
%   \left( \frac{4 \zeta}{1-z^2} \right)^{1/4}
%   \left\{
%     \mathrm{Ai}( \nu^{2/3} \zeta ) \left(1+O\left(\frac{1}{\nu^{2}}\right)\right)
%     +
%     \frac{\mathrm{Ai}^\prime( \nu^{2/3} \zeta )}{\nu^{4/3}} \left(B_0(\zeta)+O\left(\frac{1}{\nu^{2}}\right)\right) \right\}
% \end{equation}
% \begin{equation}\label{eq:compound_asymptotic_bessel_first_order}
%   Y_{\nu}(\nu z)
%   \sim
%   -\frac{1}{\nu^{1/3}}
%   \left( \frac{4 \zeta}{1-z^2} \right)^{1/4}
%   \left\{
%     \mathrm{Bi}( \nu^{2/3} \zeta ) \left(1+O\left(\frac{1}{\nu^{2}}\right)\right)
%     +
%     \frac{\mathrm{Bi}^\prime( \nu^{2/3} \zeta )}{\nu^{4/3}} \left(B_0(\zeta)+O\left(\frac{1}{\nu^{2}}\right)\right) \right\}
% \end{equation}
% Since we are interested in the asymptotics with the argument $\nu^{2/3} \zeta$ we substitute in the above and find
% \begin{equation}
%   \xi
%   =
%   \frac{2}{3} (\nu^{2/3} \zeta)^{\frac{3}{2}}
%   =
%   \nu \frac{2}{3} \zeta^{\frac{3}{2}}
%   =
%   \nu \left( \ln \frac{1+\sqrt{1-z^2}}{z} - \sqrt{1-z^2} \right)
% \end{equation}
% which gives
% \begin{equation}\label{eq:Airy_A}
%   \mathrm{Ai}(\nu^{2/3} \zeta)
%   \sim
%   \frac{e^{-\xi}}{2\sqrt{\pi}\nu^{1/6} \zeta^{1/4}}\sum_{k=0}^{\infty}(-1)^{k}\frac{u_{k}}{\xi^{k}}
% \end{equation}
% \begin{equation}\label{eq:Airy_A_prime}
%   \mathrm{Ai}^\prime(\nu^{2/3} \zeta)
%   \sim
%   -\frac{\nu^{1/6} \zeta^{1/4} e^{-\xi}}{2\sqrt{\pi}}\sum_{k=0}^{\infty}(-1)^{k}\frac{v_{k}}{\xi^{k}}
% \end{equation}
% \begin{equation}\label{eq:Airy_B}
%   \mathrm{Bi}(\nu^{2/3} \zeta)
%   \sim
%   \frac{e^{\xi}}{\sqrt{\pi}\nu^{1/6} \zeta^{1/4}}\sum_{k=0}^{\infty}\frac{u_{k}}{\xi^{k}}
% \end{equation}
% \begin{equation}\label{eq:Airy_B_prime}
%   \mathrm{Bi}^\prime(\nu^{2/3} \zeta)
%   \sim
%   \frac{\nu^{1/6} \zeta^{1/4}e^{\xi}}{\sqrt{\pi}}\sum_{k=0}^{\infty}\frac{v_{k}}{\xi^{k}}
% \end{equation}
% Hence
% \begin{equation*}
%   J_{\nu}(\nu z)
%   \sim
%   \frac{e^{-\xi}}{2\sqrt{\pi}}
%   \frac{1}{\nu^{1/3}}
%   \left( \frac{4 \zeta}{1-z^2} \right)^{1/4}
%   \left\{
%     \frac{1}{\nu^{1/6} \zeta^{1/4}}
%     \sum_{k=0}^{\infty}(-1)^{k}\frac{u_{k}}{\xi^{k}}
%     \left(1+O\left(\frac{1}{\nu^{2}}\right)\right)
%     - \frac{\zeta^{1/4}}{\nu^{7/6}} \sum_{k=0}^{\infty}(-1)^{k}\frac{v_{k}}{\xi^{k}}
%     \left(B_0(\zeta)+O\left(\frac{1}{\nu^{2}}\right)\right)
%   \right\}
% \end{equation*}
% \begin{equation*}
%   Y_{\nu}(\nu z)
%   \sim
%   -\frac{e^{\xi}}{\sqrt{\pi}}\frac{1}{\nu^{1/3}}
%   \left( \frac{4 \zeta}{1-z^2} \right)^{1/4}
%   \left\{
%     \frac{1}{\nu^{1/6} \zeta^{1/4}}\sum_{k=0}^{\infty}\frac{u_{k}}{\xi^{k}}
%     \left(1+O\left(\frac{1}{\nu^{2}}\right)\right)
%     +
%     \frac{\zeta^{1/4}}{\nu^{7/6}} \sum_{k=0}^{\infty}\frac{v_{k}}{\xi^{k}}
%     \left(B_0(\zeta)+O\left(\frac{1}{\nu^{2}}\right)\right)
%   \right\}
% \end{equation*}
% Note that by Taylor
% \begin{equation*}
%   \frac{1+\frac{b_0}{n+1}}{1+\frac{b_0}{n}} = 1-\frac{b_0}{n^2} + \text{h.o.t.}
% \end{equation*}
% As in the Dunster Paper with the above we find
% \begin{equation*}
%   \frac{Y_{n+1}(x)}{Y_{n}(x)}
%   =
%   \exp((n+1) \ln() - n \ln()) \left(\frac{n^2 - x^2}{(n+1)^2-x^2}\right)^{1/4}\left(1-\frac{b_0}{n^2}\right)
% \end{equation*}
% Taylor give without writing down higher order terms
% \begin{align*}
%   \exp((n+1) \ln() - n \ln()) &= (\lambda + \sqrt{\lambda^2 - 1})\left(1 + \frac{1}{2n} - \frac{3k^2}{4n^3} + \text{h.o.t.} \right) \\
%   \left(\frac{n^2 - x^2}{(n+1)^2-x^2}\right)^{1/4} &= 1 - \frac{1}{2n} - \frac{k^2}{2n^3} + \text{h.o.t.}
% \end{align*}
% Hence, multiplying the above we find, up to higher order terms
% \begin{align*}
%   \frac{Y_{n+1}(x)}{Y_{n}(x)}
%   &=
%   (\lambda + \sqrt{\lambda^2 - 1}) \left(1 + \frac{1}{2n} - \frac{3k^2}{4n^3} \right) \left( 1 - \frac{1}{2n} - \frac{k^2}{2n^3} \right) \left(1-\frac{b_0}{n^2}\right)\\
%   &=
%   (\lambda + \sqrt{\lambda^2 - 1}) \left(1 - \frac{1}{4n^2} + O(\frac{k^2}{n^3}) \right) \left(1-\frac{b_0}{n^2}\right)
% \end{align*}
%\begin{lemma}[Estimates for the analytic part]
%  We have for $0 \leq \nu \leq \mu$
%  \begin{equation*}
%    J_\nu^2(x) + Y_\nu^2(x) \leq J_\mu^2(x) + Y_\mu^2(x)
%  \end{equation*}
%\end{lemma}
%}


==> 10_08_heterogeneous_helmholtz_abc_analytic_regularity.tex <==
\section{Analytic regularity for second order absorbing boundary conditions}
\label{section:analytic_regularity_second_order_abcs}
%-----------------------------
The present section develops similar results as~\cite[Sec.~{5.5}]{melenk02}
for a model problem with second order boundary conditions.
We start by introducing general notation:
For $d \geq 2$ and $R > 0$ let $B_R \subset \mathbb{R}^d$ denote the ball of radius $R$ with center in the origin.
Let $B_R^+\subset \mathbb{R}^d$
be a half ball with radius $R$,
i.e., $B_R^+ = \{x \in B_R \colon x_d > 0 \}$.
Furthermore, let $\Gamma_R:= \{ x \in B_R \colon x_d = 0  \}$.
We consider functions $u$ that satisfy
\begin{equation}\label{eq:problem-half-ball}
	\begin{alignedat}{2}
		-\nabla \cdot (A \nabla u) & = f \quad   &&\text{in } B_R^+,\\
		\partial_{n_A} u + \alpha \nabla_\Gamma \cdot (A_\Gamma \nabla_\Gamma u) & = \alpha^{1/2} g + G \quad   &&\text{on } \Gamma_R,
	\end{alignedat}
\end{equation}
with the conormal derivative $\partial_{n_A} u = \normal \cdot (A \nabla u)$.
We assume that solutions $u$ of \eqref{eq:problem-half-ball} satisfy
\begin{align}
\label{eq:weak-formulation}
a(u,v)& := \int_{B_R^+} (A \nabla u) \cdot \nabla \overline{v} + \alpha \int_{\Gamma_R} (A_\Gamma \nabla_\Gamma u) \cdot \nabla_\Gamma \overline{v}  \\
\nonumber
& \qquad = \int_{B_R^+} f \overline{v} + \int_{\Gamma_R} (\alpha^{1/2} g + G ) \overline{v} \qquad \forall v \in C^\infty_0(B_R^+).
\end{align}
To describe the parameter $\alpha$, it is convenient to introduce, for fixed $\theta > 0$,  the sector
$$
\mathcal{S}_\theta := \{\alpha \in \mathbb{C}\,|\, |\operatorname{arg} \alpha | \leq \pi -\theta \}.
$$
%---------------------------------------------------------
\subsection{The shift theorem in tangential direction}
%---------------------------------------------------------
The proof of Lemma~\ref{lemma:H2-regularity} uses the well-established difference quotients method of Nirenberg that can be found, e.g.,
in~\cite[Sec.~{6.3}]{evans98}.  For $j \in \{1,\ldots,d-1\}$, the $j$-th unit vector $e_j \in \mathbb{R}^d$,
and $h \in \mathbb{R}\setminus \{0\}$ we introduce the translation operator $\tau^h_j$ by $(\tau^h_j v)(x) = v(x +h e_j)$ and the
difference quotient $(D^h_j v)(x) = h^{-1}( v(x+h e_j) - v(x))$. Inspection of the proof of~\cite[Sec.~{5.8.2}, Thm.~{3}]{evans98}
shows that for fixed $0 < r_1< r_2$
\begin{equation}
\label{eq:evans-1}
\partial_{x_j} v \in L^2(B_{r_2}) \quad \Longrightarrow \quad \|D^h_j v\|_{L^2(B_{r_1})} \leq \|\partial_{x_j} v\|_{L^2(B_{r_2}) }
\quad \forall |h| < r_2 - r_1,
\end{equation}
as well as
\begin{equation}
  \label{eq:evans-2}
  \|D^h_j v \|_{L^2(B_{r_1})} \leq C_v \quad \forall |h| \leq r_2 - r_1 \quad \Longrightarrow \quad \|\partial_{x_j} v \|_{L^2(B_{r_1})} \leq C_v.
\end{equation}

\begin{lemma}
  \label{lemma:H12}
   Let $G$, $u \in H^{1}(B_R^+)$.
   Let $r$, $\delta>0$
   with $r+\delta < R$ be given.
   Let $\chi \in C^\infty_0(\mathbb{R}^d;\mathbb{R})$
   be a cut-off function
   with $\operatorname{supp} \chi \subset B_{r+\delta/2}$
   and $\chi \equiv 1$ on $B_r$.
   Then there exists a constant $C > 0$ depending only on the spatial dimension, such that
   \begin{align*}
     &\left| \int_{\Gamma_R} G  D^{-h}_{x_j} (\chi D^h_{x_j} u)\right|
     \leq  \\
     & \qquad C \left( \delta^{-1} \|G\|_{L^2(B^+_{r+\delta})} + \|\nabla G\|_{L^2(B^+_{r+\delta})}\right)
     \left(\delta^{-1} \|\nabla u\|_{L^2(B^+_{r+\delta})} + \|\chi \nabla D^{h}_{x_j} u\|_{L^2(B^+_{r+\delta})}\right).
   \end{align*}
\end{lemma}
%
%
\begin{proof}
Let $\chi'$ be another cut-off function with $\operatorname{supp} \chi' \subset B_{r+\delta}$,
$\chi' \equiv 1$ on $\operatorname{supp} \chi$ and $\|\nabla \chi'\|_{L^\infty} \leq C \delta^{-1}$.
Then, for $h$ sufficiently small (depending only on $r$, $\delta$)
$$
\int_{\Gamma_R} G D^{-h}_{j} (\chi D^h_{j} u) =
\int_{\Gamma_R} \chi' G  D^{-h}_{j} (\chi D^h_{j} u).
$$
Let $v = D^{-h}_{j} (\chi D^h_{j} u)$.
Scaling $B^+_R$ to a half ball of radius $1$, we denote by $\widehat G$
the scaled version of $\chi' G$ and by $\widehat v$ the scaled version of $v$.
It is also convenient to define $\psi$
as the solution of the Neumann problem $-\Delta \psi = 0$ in $B^+_1$ and $\partial_n \psi = \widehat v$ on $\partial B^+_1$.
Note that $\widehat v \equiv 0$ on $\partial B^+_1 \setminus \Gamma_1$.
Furthermore, $\int_{\Gamma_1} \widehat v = 0$ and therefore the solvability condition for the above Neumann problem is satisfied.
We then have
\begin{align*}
  R^{-(d-1)} \int_{\Gamma_R} \chi' G v
  & = \int_{\partial B^+_1}  \widehat G \widehat v
  = \int_{\partial B^+_1}  \widehat G \partial_n \psi
  = \int_{B^+_1} \nabla  \widehat G \cdot \nabla \psi  \\
  & \leq \|\nabla \widehat G\|_{L^2(B^+_1)} \|\nabla \psi\|_{L^2(B^+_1)}  \\
  & \leq R^{(1-d)/2} \|\nabla (\chi' G)\|_{L^2(B^+_R)} \|\widehat v\|_{H^{-1/2}(\partial B^+_1)}.
\end{align*}
Since $\widehat v \equiv 0$ on $\partial B^+_1 \setminus \Gamma_1$, we estimate $\|\widehat v\|_{H^{-1/2}(\partial B^+_1)} \leq C \|\widehat v\|_{H^{-1/2}(\Gamma_1)}$.
To estimate this last norm, we write $w = \chi D^h_{j} u$ and denote by $\widehat w$ the corresponding scaled function.
We  observe for $\varphi \in C^\infty_0(\Gamma_1)$ and $h$ sufficiently small (depending only on $\delta$, $r$, $R$)
\begin{align*}
  \left| \int_{\Gamma_1} (D^{-h/R}_{j} \widehat w) \varphi \right| &  =
  \left| \int_{\Gamma_1} \widehat w D^{h/R}_{j} \varphi \right|  \\
  & \leq \|\widehat w\|_{L^2(\Gamma_1)} \|D^{h/R}_{j}   \varphi\|_{L^2(\Gamma_2)}\\
  &\stackrel{(\ref{eq:evans-1})}{\leq} \|\widehat w\|_{L^2(\Gamma_1)} \|\partial_{x_j}   \varphi\|_{L^2(\Gamma_1)}\\
  &\leq \|\widehat w\|_{L^2(\Gamma_1)} \|\varphi\|_{H^1(\Gamma_1)}.
\end{align*}
Hence, $\|D^{-h/R}_{j} \widehat w\|_{H^{-1}(\Gamma_1)} \leq C \|\widehat w\|_{L^2(\Gamma_1)}$ uniformly in $h$.
Similarly, (\ref{eq:evans-1}) shows
\begin{equation*}
  \|D^{-h/R}_{x_j} \widehat w\|_{L^{2}(\Gamma_1)} \leq C \|\partial_{x_j} \widehat w\|_{L^2(\Gamma_1)} \leq C\|\widehat w\|_{H^1(\Gamma_1)}
\end{equation*}
uniformly in $h$. By interpolation, we arrive at
\begin{align*}
\|D^{-h/R}_{x_j} \widehat w\|_{H^{-1/2}(\Gamma_1)} \leq C \|\widehat w\|_{H^{1/2}(\Gamma_1)}
\leq C \|\widehat w\|_{H^1(B^+_1)}
\leq C \|\nabla \widehat w\|_{L^2(B^+_1)},
\end{align*}
where the penultimate estimate follows from the trace inequality and the last one by a Poincar\'e inequality,
which is applicable due to the support properties of $\widehat w$.
In conclusion, we arrive at
\begin{align*}
&\left|
\int_{\Gamma_R} G D^{-h}_{x_j} (\chi D^h_{x_j} u)
\right|
 \leq C  \|\nabla (\chi' G)\|_{L^2(B^+_R)} \|\nabla (\chi D^h_{x_j} u)\|_{L^2(B^+_R)}  \\
&\qquad \leq C  \left( \delta^{-1} \|G\|_{L^2(B^+_{r+\delta})} + \|\nabla G\|_{L^2(B^+_{r+\delta})} \right)\left( \delta^{-1} \|\nabla u\|_{L^2(B^+_{r+\delta})}  + \|\chi\nabla D^h_{x_j} u\|_{L^2(B^+_{r+\delta})}
\right).
\end{align*}
\end{proof}
%
%
%
\begin{lemma}
\label{lemma:H2-regularity}
Let $A \in C^1(\overline{B}_R^+)$, $A_\Gamma \in C^1(\overline{\Gamma}_R^+)$ be matrix-valued functions that are pointwise
symmetric positive definite with lower bound on the eigenvalues $\lambda_{\mathrm{min}}>0$.
Let $\alpha \in \mathcal{S}_\theta$.
Let $f \in L^2(B_R^+)$, $g \in L^2(\Gamma_R)$ and $G \in H^{1}(B_R^+)$.
Then there exists $C_{\mathrm{stab}} > 0$ depending only on $\theta$,
a lower bound on $\lambda_{\mathrm{min}}$, and an upper bound on
$\|A\|_{L^\infty} + R \| \nabla A\|_{L^\infty} +
\|A_\Gamma\|_{L^\infty} + R \| \nabla A_\Gamma\|_{L^\infty} $
such that any solution $u$ of (\ref{eq:problem-half-ball}) satisfies for all $r$, $\delta>0$
 with $r+\delta < R$
\begin{align}
\nonumber
& \|\nabla^2 u\|_{L^2(B_{r})}  +
|\alpha|^{1/2} \|\nabla^2_\Gamma u\|_{L^2(\Gamma_{r})}
\leq \\
\label{eq:lemma:H2-regularity-100}
& \quad C_{\mathrm{stab}}
\Bigl(\|f\|_{L^2(B_{r+\delta}^+)} + \|g\|_{L^2(\Gamma_{r+\delta})}  + \delta^{-1} \|G\|_{L^2(B^+_{r+\delta})} + \|\nabla G\|_{L^2(B^+_{r+\delta})}  \\
\nonumber
&  \qquad \qquad \mbox{} +
\delta^{-1} \|\nabla u\|_{L^2({B_{r+\delta}^+})} +
|\alpha|^{1/2} \delta^{-1} \|\nabla_\Gamma  u\|_{L^2(\Gamma_{r+\delta})}
\Bigr).
\end{align}
\end{lemma}
\begin{proof}

\emph{Step 1:}
  A calculation reveals that $\alpha \in S_{\theta}$
  implies the existence of $c_{\mathrm{coer}} > 0$ such that
\begin{align}
\label{eq:coer}
| y_1 + \alpha y_2 | & \ge c_{\mathrm{coer}} (y_1 + |\alpha| y_2) \qquad \forall y_1, y_2 \ge 0.
\end{align}
\emph{Step 2:}
Let $\chi \in C^\infty_0(\mathbb{R}^d;\mathbb{R})$
be a cut-off function
with $\operatorname{supp} \chi \subset B_{r+\delta/2}$
and $\chi \equiv 1$ on $B_r$.
We assume furthermore
$\|\nabla \chi\|_{L^\infty} \leq C \delta^{-1}$,
and $\partial_{n_A} \chi = 0$ on $\Gamma_R$,
see~\cite[Lemma~{5.5.21}]{melenk02} for a similar construction.
For $h$ sufficiently small,
we select the test function $v = - D^{-h}_j \chi^2 D^h_j u$ in
\eqref{eq:weak-formulation}  and get
\begin{align}
  \label{eq:lemma:H2-regularity-10}
  a(u,-D^{-h}_j \chi^2 D^h_j u) &= - \int_{B_R^+} f D^{-h}_j \chi^2 D^h_j \overline{u} - \int_{\Gamma_R} (\alpha^{1/2} g+G) D^{-h}_j \chi^2 D^h_j \overline{u}.
\end{align}
We treat the left-hand and the right-hand side separately.
We proceed as in the proof of~\cite[Sec.~{6.3}, Thm.~{1}]{evans98}.
We have
\begin{align*}
  -\int_{B_R^+} (A \nabla u) \, \cdot &\nabla (D^{-h}_j \chi^2 D^h_j \overline{u})
  = \int_{B_R^+} D^h_j (A \nabla u) \cdot \nabla (\chi^2 D^h_j \overline{u}) \\
  &= \int_{B_R^+} ((\tau^h_j A) (D^h_j \nabla u) + (D^h_j A) \nabla u) \cdot \nabla (\chi^2 D^h_j \overline{u})  \\
  &= \int_{B_R^+} ((\tau^h_j A) (D^h_j \nabla u) + (D^h_j A) \nabla u) \cdot \left(
   \chi^2 \nabla D^h_j \overline{u} + 2\chi \nabla \chi D^h_j \overline{u} \right) \\
  &= \int_{B^+_R} \chi^2 ((\tau^h_j A) \nabla D^h_j u) \cdot \nabla D^h_j \overline{u} + R_{\mathrm{vol}}
\end{align*}
with $R_{\mathrm{vol}}$ given by
\begin{equation*}
   R_{\mathrm{vol}} =
   \int_{B_R^+} (\tau^h_j A) (D^h_j \nabla u) 2\chi \nabla \chi D^h_j \overline{u}
   + (D^h_j A) \nabla u \cdot
   \left(
    \chi^2 \nabla D^h_j \overline{u} +
    2\chi \nabla \chi D^h_j \overline{u}
     \right).
\end{equation*}
Hence, we can estimate
\begin{align*}
|R_{\mathrm{vol}}| &\leq
C \delta^{-1} \|A\|_{L^\infty} \|\chi \nabla D^h_j u\|_{L^2(B_R^+)} \|D^h_j u\|_{L^2(B^+_{r+\delta/2})}  \\
& \qquad \qquad+ C \|\nabla A\|_{L^\infty} \|\nabla u\|_{L^2(B^+_{r+\delta/2})} \|\chi \nabla D^h_j u\|_{L^2(B^+_R)} \\
& \qquad \qquad+ C \delta^{-1} \|\nabla A\|_{L^\infty} \|\nabla u\|_{L^2(B^+_{r+\delta/2})} \|D^h_j u\|_{L^2(B^+_{r+\delta/2})}.
%\\
%&
%\quad \stackrel{(\ref{eq:evans-1}), C.S.}{\ge} \frac{1}{2} \lambda_{\mathrm{min}} \|\chi \nabla D^j_j u\|^2_{L^2(B^+_R)}
%-  C \left(\lambda_{\mathrm{min}}^{-1} \|A\|^2_{L^\infty} + \delta^2 \lambda_{\mathrm{min}}^{-1} \|\nabla A\|^2_{L^\infty} + \delta \|\nabla A\|_{L^\infty} \right) \delta^{-2} \|\nabla u\|^2_{L^2(B^+_{r+\delta})}
\end{align*}
Analogously, we get
\begin{align*}
  -\int_{\Gamma_R} (A_\Gamma \nabla_\Gamma) \, \cdot \nabla_\Gamma D^{-h}_j \chi^2 D^h_j \overline{u} =
  \int_{\Gamma_R} \chi^2 ((\tau^h_j A_\Gamma) \nabla_\Gamma D^h_j u) \cdot \nabla_\Gamma D^h_j u + R_{\mathrm{bnd}}
\end{align*}
with
\begin{align*}
|R_{\mathrm{bnd}}| &\leq
C \delta^{-1} \|A_\Gamma\|_{L^\infty} \|\chi \nabla_\Gamma D^h_j u\|_{L^2(\Gamma_R)} \|D^h_j u\|_{L^2(\Gamma_{r+\delta/2})}\\
& \qquad \qquad + C \|\nabla A_\Gamma\|_{L^\infty} \|\nabla_\Gamma u\|_{L^2(\Gamma_{r+\delta})} \|\chi \nabla_\Gamma D^h_j u\|_{L^2(\Gamma_R)} \\
& \qquad \qquad + C \delta^{-1} \|\nabla A_\Gamma\|_{L^\infty} \|\nabla_\Gamma u\|_{L^2(\Gamma_{r+\delta/2})} \|D^h_j u\|_{L^2(\Gamma_{r+\delta/2})}.
\end{align*}
For the right-hand side of \eqref{eq:lemma:H2-regularity-10}, we get with \eqref{eq:evans-1} applied to $v = -D^{-h}_j \chi^2 D^h_j u$ and Lemma~\ref{lemma:H12}
\begin{align*}
  &\left|
    \int_{B^+_R} f D^{-h}_j \chi^2 D^h_j \overline{u}
  \right|
   \leq C \|f\|_{L^2(B^+_{r+\delta/2})}
  \left(
  \delta^{-1} \|D^h_j u\|_{L^2(B^+_{r+\delta/2})} + \|\chi \nabla D^h_j u\|_{L^2(B^+_{R})}
  \right), \\
  &\left| \int_{\Gamma_R}  g D^{-h}_j \chi^2 D^h_j \overline{u}
  \right|
   \leq C  \|g\|_{L^2(\Gamma_{r+\delta/2})} \left(
  \delta^{-1} \|D^h_j u\|_{L^2(\Gamma_{r+\delta/2})} + \|\chi \nabla_\Gamma D^h_j u\|_{L^2(\Gamma_{R})} \right),  \\
  &\left| \int_{\Gamma_R} G D^{-h}_j \chi^2 D^h_j \overline{u} \right| =
  \left| \int_{\Gamma_R} D^h_j G  \chi^2 D^h_j \overline{u}  \right|  \\
  & \qquad \leq
  C \left(\delta^{-1} \|G\|_{L^2(B^+_{r+\delta})} + \|\nabla G\|_{L^2(B^+_{r+\delta})} \right)
    \left(\delta^{-1} \|\nabla u\|_{L^2(B^+_{r+\delta})} + \|\chi \nabla D^h_j u\|_{L^2(B^+_{r+\delta})} \right).
\end{align*}
\emph{Step 3:}
Using \eqref{eq:coer} we get
\begin{align*}
  & c_{\mathrm{coer}} \left( \int_{B^+_R} \chi^2 ((\tau^h_j A) \nabla D^h_j u ) \cdot \nabla D^h_j \overline{u} +
  |\alpha|
  \int_{\Gamma_R} \chi^2 ((\tau^h_j A) \nabla_\Gamma D^h_j u )\cdot \nabla_\Gamma D^h_j \overline{u} \right)  \\
  & \qquad \leq |a(u,-D^{-h}_j \chi^2 D^h_j u) - R_{\mathrm{vol}} - \alpha R_{\mathrm{bnd}} | \\
  & \qquad \leq
  \left| \int_{B^+_R} f D^{-h}_j \chi^2 D^h_j \overline{u} \right|
  + \left| \int_{\Gamma_R} (\alpha^{1/2} g+G) D^{-h}_j \chi^2 D^h_j \overline{u}
  \right| + |R_{\mathrm{vol}}| + |\alpha| |R_{\mathrm{bnd}}|.
\end{align*}
Using the lower bound for $A$ and $A_\Gamma$ and the above estimates together with (\ref{eq:evans-1}) we find
\begin{align*}
c_{\mathrm{coer}} \lambda_{\mathrm{min}}
& \left( \|\chi \nabla D^h_j u\|^2_{L^2(B^+_R)} + |\alpha| \|\chi \nabla_\Gamma D^h_j u\|^2_{L^2(\Gamma_R)}\right)
\leq   \\
C \Bigl(
& \|f\|_{L^2(B^+_{r+\delta})} \delta^{-1} \|\partial_{x_j} u\|_{L^2(B_{r+\delta})} + \|f\|_{L^2(B^+_{r+\delta})} \|\chi \nabla D^h_j u\|_{L^2(B^+_R)}  \\
& +  \|g\|_{L^2(B^+_{r+\delta})} \delta^{-1} |\alpha|^{1/2} \|\partial_{x_j} u\|_{L^2(\Gamma_{r+\delta})}
                +  \|g\|_{L^2(\Gamma_{r+\delta})} |\alpha|^{1/2} \|\chi \nabla_\Gamma D^h_j u\|_{L^2(\Gamma_R)}  \\
& +  \left(\delta^{-1} \|G\|_{L^2(B^+_{r+\delta})} + \|\nabla G\|_{L^2(B^+_{r+\delta})} \right)
    \left(\delta^{-1} \|\nabla u\|_{L^2(B^+_{r+\delta})} + \|\chi \nabla D^h_j u\|_{L^2(B^+_{r+\delta})} \right) \\
& + (\|A\|_{L^\infty} + \delta \|\nabla A\|_{L^\infty}) \delta^{-1} \|\nabla u\|_{L^2(B^+_{r+\delta})} \|\chi \nabla D^h_j u\|_{L^2(B^+_R)} \\
&  + \delta \|\nabla A\|_{L^\infty} \delta^{-2} \|\nabla u\|^2_{L^2(B^+_{r+\delta} )} \\
&  + (\|A_\Gamma\|_{L^\infty} + \delta \|\nabla A_\Gamma\|_{L^\infty})
    |\alpha| \delta^{-1} \|\nabla_\Gamma u\|_{L^2(\Gamma_{r+\delta})} \|\chi \nabla_\Gamma D^h_j u\|_{L^2(\Gamma_R)} \\
&   + \delta \|\nabla A_\Gamma\|_{L^\infty} |\alpha| \delta^{-2} \|\nabla_\Gamma u\|^2_{L^2(\Gamma_{r+\delta} )}
\Bigr).
\end{align*}
The Cauchy-Schwarz inequality with epsilon allows us to absorb the terms
$\|\chi \nabla D^h_j u\|_{L^2(B^+_R)}$  and $\|\chi \nabla_\Gamma D^h_j u\|_{L^2(\Gamma_R)}$
from the right-hand side into the left-hand side
and we get
\begin{align*}
  \frac{1}{2} c_{\mathrm{coer}} \lambda_{\mathrm{min}}
  & \left( \|\chi \nabla D^h_j u\|^2_{L^2(B^+_R)} + |\alpha| \|\chi \nabla_\Gamma D^h_j u\|^2_{L^2(\Gamma_R)}\right)
  \leq   \\
  C \Bigl(
  & \|f\|_{L^2(B^+_{r+\delta})} \delta^{-1} \|\partial_{x_j} u\|_{L^2(B_{r+\delta})} + \lambda_{\mathrm{min}}^{-1} \|f\|^2_{L^2(B^+_{r+\delta})}  \\
  & +  \|g\|_{L^2(B^+_{r+\delta})} \delta^{-1} |\alpha|^{1/2} \|\partial_{x_j} u\|_{L^2(\Gamma_{r+\delta})}
    + \lambda_{\mathrm{min}}^{-1} \|g\|^2_{L^2(\Gamma_{r+\delta})} \\
  & +   \left(\delta^{-1} \|G\|_{L^2(B^+_{r+\delta})} + \|\nabla G\|_{L^2(B^+_{r+\delta})} \right)
      \delta^{-1} \|\nabla u\|_{L^2(B^+_{r+\delta})} \\
  & +  R^2 \lambda_{\mathrm{min}}^{-1} \left(\delta^{-1} \|G\|_{L^2(B^+_{r+\delta})} + \|\nabla G\|_{L^2(B^+_{r+\delta})} \right)^2 \\
  & + \lambda_{\mathrm{min}}^{-1} (\|A\|_{L^\infty} + \delta \|\nabla A\|_{L^\infty})^2 \delta^{-2} \|\nabla u\|^2_{L^2(B^+_{r+\delta})} \\
  &  + \delta \|\nabla A\|_{L^\infty} \delta^{-2} \|\nabla u\|^2_{L^2(B^+_{r+\delta} )} \\
  & + \lambda_{\mathrm{min}}^{-1} (\|A_\Gamma\|_{L^\infty}
     + \delta \|\nabla A_\Gamma\|_{L^\infty})^2 |\alpha| \delta^{-2} \|\nabla_\Gamma u\|^2_{L^2(\Gamma_{r+\delta})} \\
  & + \delta \|\nabla A_\Gamma\|_{L^\infty} |\alpha| \delta^{-2} \|\nabla_\Gamma u\|^2_{L^2(\Gamma_{r+\delta} )}
  \Bigr).
\end{align*}
From \eqref{eq:evans-2},
we get in the limit $h \rightarrow 0$
that
$\nabla \partial_{x_j} u \in L^2(B^+_r)$ and
$\nabla_\Gamma  \partial_{x_j} u \in L^2(\Gamma^+_r)$ together with
\begin{align}
	\nonumber
  & \|\nabla \nabla_{x'} u\|_{L^2(B_{r})}  +
  |\alpha|^{1/2} \|\nabla_\Gamma \nabla_{x'} u\|_{L^2(\Gamma_{r})}
  \leq \\
	\label{eq:lemma:H2-regularity-200}
  & \quad C_{\mathrm{stab}}
  \Bigl(\|f\|_{L^2(B_{r+\delta}^+)} + \|g\|_{L^2(\Gamma_{r+\delta})}  + \delta^{-1} \|G\|_{L^2(B^+_{r+\delta})} + \|\nabla G\|_{L^2(B^+_{r+\delta})} \\
  \nonumber
  &  \qquad \qquad \mbox{} +
  \delta^{-1} \|\nabla u\|_{L^2({B_{r+\delta}^+})} +
  |\alpha|^{1/2} \delta^{-1} \|\nabla_\Gamma  u\|_{L^2(\Gamma_{r+\delta})}
  \Bigr)
\end{align}
with $C_{\mathrm{stab}} > 0$ depending only on $\theta$,
a lower bound on $\lambda_{\mathrm{min}}$, and an upper bound on
$\|A\|_{L^\infty} + R \| \nabla A\|_{L^\infty} +
\|A_\Gamma\|_{L^\infty} + R \| \nabla A_\Gamma\|_{L^\infty} $.
\\
\noindent
\emph{Step 4:} We complete the proof by controlling $\|\partial_{x_d}^2 u\|_{L^2(B^+_{r})}$.
This follows from the differential equation
$$
- A_{dd} \partial_{x_d}^2 u  = f + \sum_{i, j=1}^d (\partial_{x_i} A_{ij}) \partial_{x_j} u - \sum_{(i,j) \ne (d,d)} A_{ij} \partial_{x_i}\partial_{x_j} u.
$$
We have
$ A_{dd}  = e_d^\top A e_d \ge \lambda_{\mathrm{min}}$ and therefore
\begin{align*}
  \lambda_{\mathrm{min}} \|\partial_{x_d}^2 u\|_{L^2(B^+_r)} & \leq \|f\|_{L^2(B^+_r)} + C \delta \|\nabla A\|_{L^\infty} \delta^{-1} \|\nabla u\|_{L^2(B^+_r)}
  + \|A\|_{L^\infty} \|\nabla \nabla_{x'} u\|_{L^2(B^+_r)}.
\end{align*}
Noting $\frac{\|A\|_{L^\infty}}{\lambda_{\mathrm{min}}} \ge 1$ together with \eqref{eq:lemma:H2-regularity-200}
concludes the proof.


\end{proof}
%--------------------------------------------------
\subsection{Control of the tangential derivatives}
%--------------------------------------------------
For functions
$v = (v_i)_{i \in \mathbf{I}}$, ($\mathbf{I}$
some finite index set)
defined on $\mathbb{R}^d$ we introduce the notation
\begin{equation}
  |\nabla^p v|^2 = \sum_{i \in \mathbf{I}} \sum_{\balpha \in \mathbb{N}_0^d\colon |\balpha| = p} \frac{|\balpha|!}{\balpha!} |D^{\balpha} v_i|^2.
\end{equation}
Analogously, the notation $|\nabla^p_{x'} v|$ for $x' \in \mathbb{R}^{d-1}$ indicates that $\balpha \in \mathbb{N}^{d-1}$ in the sum.
We proceed as described, e.g., in~\cite[Sec.~{5.5.3} and~{5.5.4}]{melenk02}.
We write $\nabla_{x'}$ for the tangential
derivatives in contrast to~\cite[Sec.~{5.5.3}]{melenk02},
where $\nabla_x$ denotes the tangential derivatives and introduce
%\begin{align*}
%M^\prime_{R,p,\alpha}(f,g) &:= \frac{1}{p!} \sup_{R/2 \leq r < R} (R - r)^{p+2} \left( \|\nabla^p_x f\|_{L^2(B^+_r)} + |\alpha|^{-1/2}\|\nabla^p_x  g\|_{L^2(\Gamma_r)}\right)\\
%N^\prime_{R,p,\alpha}(v) &:=
%\begin{cases}
%\frac{1}{p!} \sup_{R/2 \leq r < R} (R - r)^{p+2} \left( \|\nabla^2 \nabla^p_x v\|_{L^2(B^+_r)} + |\alpha|^{1/2} \|\nabla^{p+2}_x v\|_{L^2(\Gamma_r)}\right),
%& \mbox{ if $p \ge 0$}  \\
%\sup_{R/2 \leq r < R} (R - r)^{p+2} \left( \|\nabla^2 \nabla^p v\|_{L^2(B^+_r)} + |\alpha|^{1/2} \|\nabla^{p+2}_x v\|_{L^2(\Gamma_r)}\right),
%& \mbox{ if $p = -1$, $-2$}
%\end{cases}
%\end{align*}
\begin{align*}
M^\prime_{R,p}(f) &:= \frac{1}{p!} \sup_{R/2 \leq r < R} (R - r)^{p+2} \|\nabla^p_{x'} f\|_{L^2(B^+_r)},  \\
M^\prime_{R,p,\Gamma}(g) &:= \frac{1}{p!} \sup_{R/2 \leq r < R} (R - r)^{p+2} \|\nabla^p_{x'} g\|_{L^2(\Gamma_r)},   \\
N^\prime_{R,p}(v) &:=
\begin{cases}
\frac{1}{p!} \sup_{R/2 \leq r < R} (R - r)^{p+2}  \|\nabla^2 \nabla^p_{x'} v\|_{L^2(B^+_r)}
& \mbox{ if $p \ge 0$},  \\
\sup_{R/2 \leq r < R} (R - r)^{p+2} \|\nabla^{2+p} v\|_{L^2(B^+_r)}
& \mbox{ if $p = -1$, $-2$},
\end{cases}
\\
N^\prime_{R,p,\Gamma}(v) &:=
\begin{cases}
\frac{1}{p!} \sup_{R/2 \leq r < R} (R - r)^{p+2}  \|\nabla^{p+2}_{x'} v\|_{L^2(\Gamma_r)}
\qquad \mbox{ for $p \ge 0 $}  , \\
\sup_{R/2 \leq r < R} (R - r)^{p+2}  \|\nabla^{p+2}_{x'} v\|_{L^2(\Gamma_r)}
\qquad \mbox{ for $p =-2$, $-1 $},
\end{cases}
\\
H_{R,p}(v)  &  := \frac{1}{[p-1]!} \sup_{R/2 \leq r < R} (R-r)^{p+1}
\!\!\left[  \|\nabla_{x'}^{p} v\|_{L^{2}(B^{+}_{r})} + \frac{R-r}{[p]}
\|\nabla^{p}_{x'} \nabla v\|_{L^{2}(B^{+}_{r})}\right],
\end{align*}
where
\begin{equation*}
[p]!:= \max\{p,1\}!.
\end{equation*}
%We need commutators:
%\begin{lemma}
%\label{lemma:commutator}
%For vector-valued $\mathbf{a}$ and matrices $A$:
%\begin{align}
%\label{eq:lemma:commutator-10}
%\left\{ \sum_{|\balpha| = p} \frac{|\balpha|!}{\balpha!} |D^{\balpha}_{x'} \nabla \cdot (A \nabla v) - \nabla \cdot (A \nabla D^\balpha_{x'} v)|^2\right\}^{1/2}
%&\leq \sum_{q=1}^{p+1}\binom{p+1}{q} |\nabla^q _{x'} A| | \nabla^{p-q}_{x'} \nabla^2 v|, \\
%\label{eq:lemma:commutator-20}
%\left\{ \sum_{|\balpha| = p} \frac{|\balpha|!}{\balpha!} |D^{\balpha}_{x'} (\mathbf{a} \cdot \nabla v)  - (\mathbf{a} \cdot \nabla D^\balpha_{x'} v)|^2\right\}^{1/2}
%& \leq \sum_{q=1}^{p}\binom{p}{q} |\nabla^q _{x'} \mathbf{a}| | \nabla^{p-q}_{x'} \nabla v|, \\
%\end{align}
%\end{lemma}
%\begin{proof}
%(\ref{eq:lemma:commutator-10}) is shown in~\cite[Lemma~{5.5.15}]{melenk02} and
%(\ref{eq:lemma:commutator-20}) in~\cite[Lemma~{A.1.4}]{melenk02}.
%\end{proof}
Analogous to~\cite[Lemmas~{5.5.15} and~{5.5.23}]{melenk02} is
\begin{lemma}
\label{lemma:5.5.15}
Let $p \in \mathbb{N}_0$.
Let $A \in C^{p+1}(\overline{B}_R^+)$, $A_\Gamma \in C^{p+1}(\overline{\Gamma}_R^+)$
be matrix-valued functions that are pointwise
symmetric positive definite with lower bound on the eigenvalues $\lambda_{\mathrm{min}}>0$.
Let $f \in H^{p}(B_R^+)$, $g \in H^{p}(\Gamma_R^+)$, $G \in H^{p+1}(B_R^+)$ and $\alpha \in \mathcal{S}_\theta$.
There exists a constant $C_B >0$ depending only on the same quantities as the constant $C_{\mathrm{stab}}$ in Lemma~\ref{lemma:H2-regularity} such that
\begin{align*}
  & N^\prime_{R,p}(u) + |\alpha|^{1/2} N^\prime_{R,p,\Gamma}(u)
  \leq C_B
  \Bigg\{
    M^\prime_{R,p}(f)  + M^\prime_{R,p,\Gamma}(g) + H_{R,p}(G)\\
    & + \sum_{q=1}^{p+1} \binom{p+1}{q} \left( \left(\frac{R}{2}\right)^q \|\nabla^q A\|_{L^\infty(B^+_R)} + \left(\frac{R}{2}\right)^{q-1} q \|\nabla^{q-1} A\|_{L^\infty(B^+_R)}
    \right) \frac{[p-q]!}{p!} N^\prime_{R,p-q}(u)  \\
    & \qquad + N^\prime_{R,p-1}(u) + N^\prime_{R,p-2}(u)  \\
    & + |\alpha|^{1/2} \Bigg( \sum_{q=1}^{p+1} \binom{p+1}{q} \left(\frac{R}{2}\right)^q \|\nabla^q_{x'} A_\Gamma\|_{L^\infty(\Gamma_R)} \frac{[p-q]!}{p!} N^\prime_{R,p-q,\Gamma}(u) \\
    & \qquad + N^\prime_{R,p-1,\Gamma}(u) + N^\prime_{R,p-2,\Gamma}(u) \Bigg)
  \Bigg\}.
\end{align*}
\end{lemma}
\begin{proof}
The proof follows the lines of the proofs of
\cite[Lemmas~{5.5.12}, {5.5.15} and~{5.5.23}]{melenk02}. We abbreviate $\mathbf{a} = A \mathbf{n}$, where $\mathbf{n}$ is the outer normal vector on $\Gamma_R$.
The derivative $D^{\balpha'}_{x'} u$ with $\balpha' \in \mathbb{N}_0^{d-1}$ satisfies
\begin{align*}
-\nabla \cdot (A \nabla D^{\balpha'}_{x'} u) & = D^{\balpha'}_{x'} f
- \{\nabla \cdot (A \nabla D^{\balpha'}_{x'} u)  - D^{\balpha'}_{x'} (\nabla \cdot (A \nabla u))\} , \\
\partial_{n_A} D^{\balpha'}_{x'} u + \alpha \nabla_\Gamma \cdot (A_\Gamma \nabla_\Gamma D^{\balpha'}_{x'} u) & = D^{\balpha'}_{x'} (\alpha^{1/2} g_1 + g_2)     \\
& \quad \mbox{} + \alpha \{\nabla_{x'} \cdot (A_\Gamma \nabla_{x'} D^{\balpha'}_{x'} u)  - D^{\balpha'}_{x'} (\nabla_{x'} \cdot (A_\Gamma \nabla_{x'} u))\}  \\
& \quad \mbox{}+ \left\{
                  (\mathbf{a} \cdot \nabla D^{\balpha'}_{x'} u)
                  -D^{\balpha'}_{x'} (\mathbf{a} \cdot \nabla u)
                  \right\}.
\end{align*}
The remainder of the proof proceeds analogously to the proof of
\cite[Lemmas~{5.5.12} and~{5.5.23}]{melenk02}
and uses Lemma~\ref{lemma:H2-regularity} with $\delta = \frac{R - r}{p+2}$.
Specifically, the terms arising from $A$, $f$, $G$ are obtained directly as in the proofs of
\cite[Lemmas~{5.5.12} and~{5.5.23}]{melenk02}. The terms arising from the Laplace-Beltrami are treated with the same arguments
as in the proof of~\cite[Lemma~{5.5.12}]{melenk02}.
\end{proof}
%-----------------------------
\subsection{Tangential control for $k$-dependent problem}
%-----------------------------
We consider the problem
\begin{equation}
\label{eq:problem-with-lower-order-terms}
\begin{alignedat}{2}
-\nabla \cdot (A \nabla u) - c k^2 u & = f \quad &&\mbox{ in $B_R^+$}, \\
\partial_{n_A} u + \alpha \nabla_\Gamma \cdot (A_\Gamma\nabla_\Gamma u) & = \alpha^{1/2} g+G + b k u
\quad &&\mbox{ on $\Gamma$}  .
\end{alignedat}
\end{equation}
For the data, we assume
\begin{subequations}
\label{eq:cond-on-data}
\begin{align}
\|\nabla^p f\|_{L^2(B^+_R)} &\leq C_f \gamma_f^p R^{-p} \max\{p+1,R k\}^p \qquad \forall p \in \mathbb{N}_0, \\
\|\nabla^p_{x'} g\|_{L^2(\Gamma_R)} &\leq C_{g} \gamma_{g}^p R^{-p}\max\{p+1,R k\}^p \qquad \forall p \in \mathbb{N}_0, \\
\|\nabla^p G\|_{L^2(B^+_R)} &\leq C_{G} \gamma_{G}^p R^{-p} \max\{p+1,R k\}^p \qquad \forall p \in \mathbb{N}_0, \\
\|\nabla^p A\|_{L^\infty(B^+_R)} &\leq C_A \gamma_A^p p! \qquad \forall p \in \mathbb{N}_0, \\
\|\nabla^p_{x'} A_\Gamma\|_{L^\infty(\Gamma_R)} &\leq C_{A_\Gamma} \gamma_{A_\Gamma}^p p! \qquad \forall p \in \mathbb{N}_0, \\
\|\nabla^p b\|_{L^\infty(B^+_R)} &\leq C_b \gamma_b^p p! \qquad \forall p \in \mathbb{N}_0, \\
\|\nabla^p c\|_{L^\infty(B^+_R)} &\leq C_c \gamma_c^p p! \qquad \forall p \in \mathbb{N}_0.
\end{align}
\end{subequations}
Additionally, we assume that
\begin{equation}
\label{eq:cond-alpha}
|\alpha|^{1/2} \leq C_{\alpha} k^{-1/2}
\end{equation}
as well as $\alpha \in S_\theta$ for some $\theta > 0$ uniformly in $k$.
\begin{theorem}
\label{thm:tangential-derivatives}
Let $R \leq 1$.
Let $f$, $g$, $G$, $A$, $A_\Gamma$, $b$ and $\alpha$ satisfy \eqref{eq:cond-on-data} and \eqref{eq:cond-alpha}, respectively.
Let $u$ solve (\ref{eq:problem-with-lower-order-terms}).
Then there exists a $K \ge 1$ depending only on
the coefficients $A$, $A_\Gamma$
of the differential operator, $\theta$, and the constants
in \eqref{eq:cond-on-data} and \eqref{eq:cond-alpha} such that for all $p \ge -1$
\begin{align}
\label{eq:thm:tangential-derivatives-10}
  N^\prime_{R,p}(u) + k^{-1/2} N^\prime_{R,p,\Gamma}(u) \leq C_u K^{p+2} \frac{\max\{p+3,Rk\}^{p+2}}{[p]!}
  \end{align}
  where
  \begin{align}
  \nonumber
  C_u & =
    \min\{1,Rk\}^2  ( k^{-2} C_f + k^{-2} C_g + C_c \|u\|_{L^2(B^+_R)})  \\ \nonumber
    & \quad  + \min\{1,Rk\} k^{-1} C_{G} (1 + \gamma_{G} R)\\
    & \quad +  \min\{1,Rk\} ( 1 + \gamma_b R) C_b \|u\|_{L^2(B^+_R)}  \\ \nonumber
   & \quad  + \min\{1,Rk\} (1 + C_b \min\{1,Rk\}) k^{-1} \|\nabla u\|_{L^2(B^+_R)}  \\ \nonumber
   & \quad
  + \min\{1,Rk\} k^{-3/2}  C_\alpha \|\nabla_\Gamma u\|_{L^2(\Gamma_R)}).
\end{align}
\end{theorem}
\begin{proof}
We will frequently use the
elementary property
$$
\min\{a,Rk\} \max\{a,Rk\} = a Rk \qquad a > 0.
$$
We first verify that \eqref{eq:thm:tangential-derivatives-10} is correct for $p = -1$, if $K \ge (1+C_\alpha^{-1})/2$.
To that end, note that
\begin{align*}
  N^\prime_{R,-1}(u)
  & \leq \frac{R}{2} \|\nabla u\|_{L^2(B_R^+)}
  = \frac{1}{2} kR k^{-1} \|\nabla u\|_{L^2(B_R^+)} \\
  &= \frac{1}{2} \max\{1,Rk\} \min\{1,Rk\} k^{-1} \|\nabla u\|_{L^2(B_R^+)} \\
  &\leq \frac{1}{2} \max\{1,Rk\} C_u, \\
  k^{-1/2} N^\prime_{R,-1,\Gamma}(u)
  & \leq  k^{-1/2} \frac{R}{2} \|\nabla_\Gamma u\|_{L^2(\Gamma_R)} \\
  & \leq  \frac{C_\alpha^{-1}}{2} \max\{1,Rk\} \min\{1,Rk\} k^{-1} k^{-1/2} C_\alpha \|\nabla_\Gamma u\|_{L^2(\Gamma_R)} \\
  & \leq  \frac{C_\alpha^{-1}}{2} \max\{1,Rk\} C_u.
\end{align*}
Hence, we have
\begin{equation*}
  N^\prime_{R,-1}(u) + k^{-1/2} N^\prime_{R,-1,\Gamma}(u) \leq \frac{1+C_\alpha^{-1}}{2} \max\{1,Rk\} C_u,
\end{equation*}
which concludes the case $p=-1$.
We next show that it is correct for $p = 0$ and then by induction for all $p \ge 1$.
To that end, we rewrite the equation as
\begin{equation*}
\begin{alignedat}{2}
-\nabla \cdot (A \nabla u) & = f + c k^2 u \quad &&\mbox{ in $B_R^+$}, \\
\partial_{n_A} u + \alpha \nabla_\Gamma \cdot (A_\Gamma\nabla_\Gamma u) & = \alpha^{1/2} g+G + b k u
\quad &&\mbox{ on $\Gamma$}  .
\end{alignedat}
\end{equation*}
For $p=0$, an application of Lemma~\ref{lemma:H2-regularity} (used with $\delta \sim R - r$) gives
\begin{align*}
& N^\prime_{R,p}(u) + k^{-1/2} N^\prime_{R,p,\Gamma}(u) \\
& \quad \leq
  C_{\mathrm{stab}}
  \Bigl(
    \frac{R^2}{4} (\|f + c k^2 u\|_{L^2(B^+_R)} + \|g\|_{L^2(\Gamma_R)}) \\
    & \qquad + \frac{R}{2} \|G + bku\|_{L^2(B^+_R)} + \frac{R^2}{4} \| \nabla (G + bku) \|_{L^2(B^+_R)} \\
    & \qquad + \frac{R}{2} \|\nabla u\|_{L^2(B^+_R)} + |\alpha|^{1/2} \frac{R}{2} \|\nabla_\Gamma u\|_{L^2(\Gamma_R)}
  \Bigr)  \\
    & \quad \leq
      C_{\mathrm{stab}}
      \Bigl(
        R^2 (\|f\|_{L^2(B^+_R)} + C_c k^2 \|u\|_{L^2(B^+_R)} + \|g\|_{L^2(\Gamma_R)}) \\
        & \qquad + R \|G\|_{L^2(B^+_R)} + R^2 \| \nabla G \|_{L^2(B^+_R)} \\
        & \qquad + R k ( 1 + \gamma_b R) C_b \|u\|_{L^2(B^+_R)} + R^2 k C_b \| \nabla u \|_{L^2(B^+_R)} \\
        & \qquad + R \|\nabla u\|_{L^2(B^+_R)} + C_\alpha k^{-1/2} R \|\nabla_\Gamma u\|_{L^2(\Gamma_R)}
      \Bigr)  \\
      & \quad \leq
        C_{\mathrm{stab}}
        \Bigl(
          R^2 (C_f + C_g + C_c k^2 \|u\|_{L^2(B^+_R)}) \\
          & \qquad + R C_G + R^2 \gamma_G C_G \\
          & \qquad + R k ( 1 + \gamma_b R) C_b \|u\|_{L^2(B^+_R)} + R^2 k C_b \| \nabla u \|_{L^2(B^+_R)} \\
          & \qquad + R \|\nabla u\|_{L^2(B^+_R)} +  R k^{-1/2} C_\alpha\|\nabla_\Gamma u\|_{L^2(\Gamma_R)}
        \Bigr)  \\
  & \quad \leq C_{\mathrm{stab}} C_u \max\{3,Rk\}^2,
\end{align*}
where the last estimate follows by similar
estimates as in the case $p=-1$.
Let us assume that (\ref{eq:thm:tangential-derivatives-10}) is correct for all $-1 \leq p' \leq p-1$ for some $p \ge 1$. We show
that it is correct for $p$ if $K$ is chosen sufficiently large. In fact, we will implicitly assume
$K >  \max\{\gamma_f,\gamma_g,\gamma_G,\gamma_c, \gamma_b\}$, so that the various geometric series below converge.

It is convenient to abbreviate
\begin{equation}
m(p):= \max\{p+3,Rk\}^{p+2}.
\end{equation}
In order to apply Lemma~\ref{lemma:5.5.15}, we have to estimate
$M^\prime_{R,p}(f - k^2 c u) $, $M^\prime_{R,p,\Gamma}(g)$  and $H^\prime(k b u) $.
Since $M^\prime_{R,p}(f - k^2 c u) \leq M^\prime_{R,p}(f) + M^\prime_{R,p}(k^2 c u)$,
we first estimate $M^\prime_{R,p}(f)$.
\begin{align*}
  M^\prime_{R,p}(f)
  &\leq \frac{1}{p!} \left(\frac{R}{2}\right)^{p+2} C_f \gamma_f^p R^{-p} \max\{p+1, Rk\}^p \\
  &\leq \frac{C_f}{4} \left(\frac{\gamma_f}{2}\right)^p R^2 \frac{1}{p!}  \max\{p+3, Rk\}^p \\
  &\leq \frac{C_f}{4} \left(\frac{\gamma_f}{2}\right)^p k^{-2} \min\{1,Rk\}^2 \frac{m(p)}{p!}.
\end{align*}
From~\cite[Lemma~{5.5.13}]{melenk02} and the induction hypothesis, we have
\begin{align*}
  M^\prime_{R,p} & (k^2 c u)
  \leq k^2 C_c
  \sum_{q=0}^p \left(\gamma_c \frac{R}{2}\right)^q \left(\frac{R}{2}\right)^2 \frac{[p-q-2]!}{(p-q)!} N^\prime_{R,p-q-2}(u) \\
  & = \frac{C_c}{4} \min\{1,Rk\}^2 \max\{1,Rk\}^2
  \sum_{q=0}^p \left(\frac{\gamma_c R}{2}\right)^q \frac{[p-q-2]!}{(p-q)!} N^\prime_{R,p-q-2}(u) \\
  & \leq \frac{C_c}{4} \min\{1,Rk\}^2 \max\{1,Rk\}^2
  \sum_{q=0}^p \left(\frac{\gamma_c R}{2}\right)^q \frac{1}{(p-q)!} K^{p-q} \max\{p-q+1,Rk\}^{p-q} C_u \\
  & = \frac{C_c}{4} \min\{1,Rk\}^2 K^p \max\{1,Rk\}^2
  \sum_{q=0}^p \left(\frac{\gamma_c R}{2K}\right)^q \frac{1}{(p-q)!} \max\{p-q+1,Rk\}^{p-q} C_u \\
  & \leq \frac{C_c}{4} \min\{1,Rk\}^2 K^p \max\{1,Rk\}^2
  \sum_{q=0}^p \left(\frac{\gamma_c R}{2K}\right)^q \frac{1}{p!} p^q \max\{p-q+1,Rk\}^{p-q} C_u \\
  & \leq \frac{C_c}{4} \min\{1,Rk\}^2 K^{p+2} \frac{m(p)}{p!} K^{-2}
  \sum_{q=0}^p \left(\frac{\gamma_c R}{2K}\right)^q C_u \\
  & \leq \frac{C_c}{4} \min\{1,Rk\}^2 K^{p+2} \frac{m(p)}{p!} \frac{K^{-2}}{1-\gamma_c R/(2K)} C_u,
\end{align*}
where the last step follows from a geometric series argument and assumes $K > \gamma_c R/2$.
Similarly, we find
\begin{align*}
  M^\prime_{R,p,\Gamma}(g)
  \leq \frac{C_g}{4} \left(\frac{\gamma_g}{2}\right)^p k^{-2} \min\{1,Rk\}^2 \frac{m(p)}{p!}.
\end{align*}
From~\cite[Lemma~{5.5.24}]{melenk02}, similar estimates to the above and the induction hypothesis, we have
\begin{align*}
  & H_{R,p}(kbu)  \leq
    C_b \frac{1}{[p]!}\frac{1}{2} \min\{1,Rk\} \times \\
    &\quad
    \Bigg\{
    \max\{p+1, Rk\}^2\sum_{q=0}^p \binom{p}{q} \left[ \left(\frac{\gamma_b R}{2}\right)^q + \left(\frac{\gamma_b R}{2}\right)^{q+1}\right]
    q! [p-q-2]!N^\prime_{R,p-q-2}(u) \\
    & \qquad \mbox{} + \max\{p+1,Rk\}\sum_{q=0}^p\binom{p}{q} \left(\frac{\gamma_b R}{2}\right)^q q! [p-q-1]! N^\prime_{R,p-q-1}(u)
    \Bigg\} \\
    &\leq \frac{C_b}{2} \min\{1,Rk\} K^{p+2} \frac{m(p)}{p!}
    \left(\frac{K^{-2}}{1-\gamma_b R/(2K)} + \frac{K^{-2} \gamma_b R/2}{1-\gamma_b R/(2K)} + \frac{K^{-1}}{1-\gamma_b R/(2K)} \right) C_u.
\end{align*}
Finally, we estimate $H_{R,p}(G)$ as at the end of the proof of~\cite[Prop.~{5.5.25}]{melenk02}
\begin{align}
  H_{R,p}(G) &\leq C_G \gamma_G^p k^{-1} \min\{1,Rk\} ( 1 + \gamma_G R) \frac{m(p)}{p!} .
\end{align}
We are now in the place to perform the induction argument.
Lemma~\ref{lemma:5.5.15} gives
\begin{align*}
  & N^\prime_{R,p}(u) + k^{-1/2} N^\prime_{R,p,\Gamma}(u) \\
  &\leq
    C_B \Bigl[ M^\prime_{R,p}(f - k^2 c u) + M^\prime_{R,p,\Gamma}(g) + H_{R,p}(G + bku) \\
    &\quad + C_A \sum_{q=1}^{p+1} \binom{p+1}{q} q!
    \left(\Bigl(\frac{R\gamma_A}{2}\Bigr)^q +  \Bigl( \frac{R \gamma_A}{2} \Bigr)^{q-1}
    \right)\frac{[p-q]!}{p!} N^\prime_{R,p-q}(u)  \\
    &\quad + N^\prime_{R,p-1}(u) + N^\prime_{R,p-2}(u) \\
    &\quad + |\alpha|^{1/2} C_{A_\Gamma} \sum_{q=1}^{p+1} \binom{p+1}{q} q! \left(\frac{R\gamma_{A_\Gamma}}{2}\right)^q \frac{[p-q]!}{p!} N^\prime_{R,p-q,\Gamma}(u) \\
    &\quad + |\alpha|^{1/2} ( N^\prime_{R,p-1,\Gamma}(u) + N^\prime_{R,p-2,\Gamma}(u))
    \Bigr] \\
  &\leq
  C_B \Bigl[
    C_f k^{-2} \min\{1,Rk\}^2 \gamma_f^p \frac{m(p)}{p!} + C_{g} k^{-2} \min\{1,Rk\}^2 \gamma_{g}^p \frac{m(p)}{p!}\\
    &\quad + \frac{C_c}{4} \min\{1,Rk\}^2 K^{p+2} \frac{m(p)}{p!} \frac{K^{-2}}{1-\gamma_c R/(2K)} C_u \\
    &\quad + C_G \gamma_G^p k^{-1} \min\{1,Rk\} (1+\gamma_G R) \frac{m(p)}{p!} \\
    &\quad + \frac{C_b}{2} \min\{1,Rk\} K^{p+2} \frac{m(p)}{p!}
    \left(\frac{K^{-2}}{1-\gamma_b R/(2K)} + \frac{K^{-2} \gamma_b R/2}{1-\gamma_b R/(2K)} + \frac{K^{-1}}{1-\gamma_b R/(2K)} \right) C_u \\
    &\quad + C_A K^{p+2} \frac{m(p)}{p!} \left( \frac{K^{-2}}{1-\gamma_A R/(2K)} + \frac{K^{-2} \gamma_A R/2}{1-\gamma_A R/(2K)}\right) C_u\\
    &\quad + K^{p+2} \frac{m(p)}{p!} \left( K^{-2} + K^{-1}\right) C_u \\
    &\quad + C_\alpha C_{A_\Gamma} K^{p+2} \frac{m(p)}{p!} \frac{K^{-2}}{1-\gamma_{A_\Gamma} R/(2K)} C_u \\
    &\quad + C_\alpha K^{p+2} \frac{m(p)}{p!} \left( K^{-2} + K^{-1}\right) C_u
    \Bigr] \\
    &\leq C_B K^{p+2} \frac{m(p)}{p!} \Bigl[
      C_f k^{-2} \min\{1,Rk\}^2 K^{-2} \left(\frac{\gamma_f}{K}\right)^p + C_g k^{-2} \min\{1,Rk\}^2  K^{-2} \left(\frac{\gamma_g}{K}\right)^p\\
      &\quad + \frac{C_c}{4} \min\{1,Rk\}^2 \frac{K^{-2}}{1-\gamma_c R/(2K)} C_u + C_G k^{-1} \min\{1,Rk\} (1+\gamma_G R) K^{-2} \left(\frac{\gamma_G}{K}\right)^p \\
      &\quad + \frac{C_b}{2} \min\{1,Rk\}
      \left(\frac{K^{-2}}{1-\gamma_b R/(2K)} + \frac{K^{-2} \gamma_b R/2}{1-\gamma_b R/(2K)} + \frac{K^{-1}}{1-\gamma_b R/(2K)} \right) C_u \\
      &\quad + C_A \left( \frac{K^{-2}}{1-\gamma_A R/(2K)} + \frac{K^{-2} \gamma_A R/2}{1-\gamma_A R/(2K)}\right) C_u + \left( K^{-2} + K^{-1}\right) C_u \\
      &\quad + C_\alpha C_{A_\Gamma} \frac{K^{-2}}{1-\gamma_{A_\Gamma} R/(2K)} C_u + C_\alpha \left( K^{-2} + K^{-1}\right) C_u
      \Bigr] \\
    &\leq C_u K^{p+2} \frac{m(p)}{p!} C_B \Bigl[ \cdots \Bigl].
\end{align*}
The induction argument is complete, once we established that there exists a sufficiently large $K$, which can be chosen uniformly in $p$ such that $C_B \Bigl[ \cdots \Bigl] \leq 1$.
This can be easily seen, since
\begin{align*}
  &C_B \Bigl[ \cdots \Bigl]
  = C_B \Bigl[
    K^{-2} \left(\frac{\gamma_f}{K}\right)^p +  K^{-2} \left(\frac{\gamma_g}{K}\right)^p + \frac{C_c}{4} \frac{K^{-2}}{1-\gamma_c R/(2K)} + K^{-2} \left(\frac{\gamma_G}{K}\right)^p \\
    &\quad + \frac{C_b}{2}
    \left(\frac{K^{-2}}{1-\gamma_b R/(2K)} + \frac{K^{-2} \gamma_b R/2}{1-\gamma_b R/(2K)} + \frac{K^{-1}}{1-\gamma_b R/(2K)} \right) \\
    &\quad + C_A \left( \frac{K^{-2}}{1-\gamma_A R/(2K)} + \frac{K^{-2} \gamma_A R/2}{1-\gamma_A R/(2K)}\right) + \left( K^{-2} + K^{-1}\right) \\
    &\quad + C_\alpha C_{A_\Gamma} \frac{K^{-2}}{1-\gamma_{A_\Gamma} R/(2K)} + C_\alpha \left( K^{-2} + K^{-1}\right)
    \Bigr],
\end{align*}
which concludes the proof.
\end{proof}
%--------------
\subsection{Control of all derivatives for $k$-dependent problems}
%--------------
Control of the derivatives $\partial_{x_d}^q$ is achieved using the differential equation. For that purpose, we introduce
\begin{align*}
N^\prime_{p,q,R}(u):= \frac{1}{[p+q]!} \sup_{R/2 \leq r  < R} (R - r)^{p+q+2} \|\nabla_{x'}^p \partial_{x_d}^{q+2} u\|_{L^2(B^+_{r})}.
\end{align*}
\begin{theorem}
\label{thm:prop.5.5.2}
Assume the hypotheses of Theorem~\ref{thm:tangential-derivatives}. Then there exist constants $K_1$, $K_2$ depending only on
the coefficients $A$, $A_\Gamma$
of the differential operator, $\theta$, and the constants
in \eqref{eq:cond-on-data} and \eqref{eq:cond-alpha} such that for all $p$, $q \in \mathbb{N}_0 \cup \{-1,-2\}$ with
$p+q \ne -2$
\begin{align}
N^\prime_{R,p,q}(u) \leq C_u K_1^{p+2} K_2^{q+2} \frac{\max\{p+q+3, Rk\}^{p+q+2} }{[p+q]!},
\end{align}
where $C_u$ is given in Theorem~\ref{thm:tangential-derivatives}.
\end{theorem}
\begin{proof}
The proof follows directly from the proof of~\cite[Prop.~{5.5.2}]{melenk02}. Namely,~\cite[Prop.~{5.5.2}]{melenk02} proceeds by induction on $q$. The induction
step relies on a) the fact that an elliptic equation in $B^+_R$ of the form studied here is considered and b) control of the tangential derivatives,
which is provided in Theorem~\ref{thm:tangential-derivatives}. Hence, the proof of~\cite[Prop.~{5.5.2}]{melenk02} applies.
\end{proof}

